Adversarial Examples in Multi-Layer Random ReLU Networks

We consider the phenomenon of adversarial examples in ReLU networks with independent gaussian parameters. For networks of constant depth and with a large range of widths (for instance, it suffices if the width of each layer is polynomial in that of any other layer), small perturbations of input vectors lead to large changes of outputs. This generalizes results of Daniely and Schacham (2020) for networks of rapidly decreasing width and of Bubeck et al (2021) for two-layer networks. The proof shows that adversarial examples arise in these networks because the functions that they compute are very close to linear. Bottleneck layers in the network play a key role: the minimal width up to some point in the network determines scales and sensitivities of mappings computed up to that point. The main result is for networks with constant depth, but we also show that some constraint on depth is necessary for a result of this kind, because there are suitably deep networks that, with constant probability, compute a function that is close to constant.

==> content/__latexindent_temp.tex <==
\subsection{Deferred Proofs}\
\label{ssec:def_proofs}

\subsubsection{Proof of \cref{lem:dist_equiv}}
\label{sssec:dis_equiv_proof}

For the first claim, we introduce the following random signed matrices, $S_i$ for $i \in [m]$ with:
\begin{equation*}
    (S_i)_{j,j} = \pm 1 \text{ with equal probability },\quad (S_i)_{j,k} = 0 \text{ otherwise}.
\end{equation*}
Now, we have from the symmetricity of the distribution:
\begin{align*}
    W_m \prod_{j = m - 1}^1  (D_j (\wt{h}_j (x)) + B_j) W_j &\overset{d}{=} W_m \lprp{\prod_{j = m - 1}^2  (D_j (\wt{h}_j (x)) + B_j) W_j} (D_1 (S_1 \wt{h}_1 (x)) + B_1) S_1 W_1 \\
    &\overset{d}{=} W_m \lprp{\prod_{j = m - 1}^2  (D_j + B_j) W_j} (D_1 (S_1 \wt{h}_1 (x)) + B_1) S_1 W_1 \\
    &\overset{d}{=} W_m \lprp{\prod_{j = m - 1}^2  (D_j + B_j) W_j} S_1 (D_1(S_1 \wt{h}_1 (x)) + B_1)  S_1 W_1 \\
    &\overset{d}{=} W_m \lprp{\prod_{j = m - 1}^2  (D_j + B_j) W_j} (D_1 (S_1 \wt{h}_1 (x)) + B_1) W_1 \\
    &\overset{d}{=} W_m \prod_{j = m - 1}^1  (D_j + B_j) W_j.
\end{align*}

For the second claim, we have:
\begin{align*}
    \norm*{\prod_{j = m}^1  (D_j (\wt{h}_j (x)) + B_j) W_j} &\overset{d}{=} \norm*{(D_m (S_m\wt{h}_m (x)) + B_m) S_m W_m \prod_{j = m - 1}^1  (D_j (\wt{h}_j (x)) + B_j) W_j} \\
    & \overset{d}{=} \norm*{S_m (D_m (S_m\wt{h}_m (x)) + B_m) S_m W_m \prod_{j = m - 1}^1  (D_j (\wt{h}_j (x)) + B_j) W_j} \\
    & \overset{d}{=} \norm*{(D_m (S_m\wt{h}_m (x)) + B_m) W_m \prod_{j = m - 1}^1  (D_j (\wt{h}_j (x)) + B_j) W_j} \\
    & \overset{d}{=} \norm*{(D_m + B_m) W_m \prod_{j = m - 1}^1  (D_j (\wt{h}_j (x)) + B_j) W_j} \\
    &\overset{d}{=} \norm*{\prod_{j = m}^1  (D_j + B_j) W_j}
\end{align*}
\qed

\subsubsection{Proof of \cref{lem:scale_pres_ml}}
\label{sssec:scale_pres_proof}

We start with the first claim of the lemma. As in \cref{lem:f_grad_conc}, we note from \cref{lem:dist_equiv}:
    \begin{gather*}
        f_i (x) = \prod_{j = i}^1 D_j(\wt{f}_j (x)) W_j x\\
        \norm*{\prod_{j = i}^1 D_j(\wt{f}_j (x)) W_j} \overset{d}{=} \norm*{\prod_{j = i}^1 D_j \wt{W}_j} \text{ where } 
        (D_i)_{j,k} = \begin{cases}
            1 & \text{w.p } 1/2 \text{ if } j = k\\
            0 & \text{otherwise}
          \end{cases}
\text{ and } \{W_i\}_{i = 1}^{\ell + 1} \overset{d}{=} \{\wt{W}_i\}_{i = 1}^{\ell + 1}.
    \end{gather*}
    Therefore, it suffices to analyze the distribution of $\prod_{j = i}^1 D_j \wt{W}_j x$. Again, we condition on the following event:
    \begin{equation*}
        \forall i \in [\ell]: \Tr D_i \geq \frac{d_i}{3}
    \end{equation*}
    which occurs with probability at least $1 - \delta / 8$. As in the
    proof of \cref{lem:f_grad_conc}, we observe the following
    distributional equivalence, when we condition on the $D_j$:
    \begin{gather*}
        \forall i \in [\ell]: \norm*{\prod_{j = i}^1 D_j \wt{W}_j x}
        \overset{d}{=} \norm*{\prod_{j = i}^1 W^\dagger_j x} \text{
        where } \forall j \in \{2, \dots, i\},\,
        W^\dagger_j \in \R^{\Tr D_j \times \Tr D_{j - 1}},\ W^\dagger_1 \in \R^{\Tr D_1 \times d} \\
        \forall j \in \{2, \dots, i\},\,
        (W^\dagger_j)_{k, :} \thicksim \mc{N} \lprp{0, I / d_{j -
        1}},\, (W^\dagger_1)_{k, :} \thicksim \mc{N} (0, I / d).
    \end{gather*}
    A recursive application of \cref{thm:tsirelson} as in the proof of \cref{lem:f_grad_conc} yields:
    \begin{equation*}
        \norm*{\prod_{j = i}^1 D_j \wt{W}_j x} \geq \lprp{\frac{1}{2}}^i
        \prod_{j = i}^1 \sqrt{\frac{d_j}{d_{j-1}}}\|x\|
    \end{equation*}
    with probability at least $1 - \delta / 16\ell^2$. A union bound over the $j$ layers concludes the proof of the first claim of the lemma.
    % \begin{align*}
    %     \norm*{\prod_{j = i}^1 D_j \wt{W}_j x} &\geq \frac{1}{2} \cdot \sqrt{\frac{d_i}{d_{i - 1}}}\norm*{\prod_{j = i - 1}^1 D_j \wt{W}_j x} && \text{Conditioning on } \prod_{j = i - 1}^1 D_j \wt{W}_j x \\ &\geq \lprp{\frac{1}{2}}^i \sqrt{d_i} && \text{By induction with probability at least } 1 - \delta / (8\ell).
    % \end{align*}
    % A union bound over the $j$ layers concludes the proof of the first claim of the lemma.

    % We will establish the second claim through a gridding based argument with some subtleties. Namely, we construct a new grid over the image of $\mb{B}(x,R)$ whenever the number of units in a hidden layer drops. With this outline in mind, we start by splitting our neural network into a series of segments. We define these segments inductively as follows:
    % \begin{equation*}
    %     i_1 = \ell, \qquad i_{j + 1} \coloneqq \argmin_{j < i_j} d_j
    % \end{equation*}
    % with segments implicitly defined by indices $\{i_j\}_{j = 1}^m$. Note $m \leq \ell$ and for $i_{j + 1} < i < i_j$, we have $d_i \geq d_{i_{j + 1}}$. We now establish the following claim inductively:
    We will establish the second claim through a gridding based argument with some subtleties. Namely, we construct a new grid over the image of $\mb{B}(x,R)$ whenever the number of units in a hidden layer drops lower than all the previous layers in the network starting from the input layer. These layers are precisely defined by the indices $i_j$ in \ref{eq:nn_dec}. We now establish the following claim inductively.
    \begin{claim}
        \label{clm:per_segmend_sp}
        Suppose for $j > 1$ and $\wt{R} \leq \dmax \cdot R$:
        \begin{equation*}
            \forall y \in \mb{B} (x, R): \norm{f_{i_j}(x) - f_{i_j} (y)} \leq \wt{R}.
        \end{equation*}
        Then:
        \begin{gather*}
            \forall i \in \{i_j + 1, \dots, i_{j - 1} - 1\}, y \in
            \mb{B} (x, R): \norm{\wt{f}_i (x) - \wt{f}_i (y)} \leq \lprp{C \ell \log
            \dmax}^{(i - i_j) / 2} \cdot \sqrt{\frac{d_i}{d_{i_j}}}
            \cdot \wt{R}, \\
            \forall y \in \mb{B} (x, R): \norm{\wt{f}_{i_{j-1}} (x) -
            \wt{f}_{i_{j-1}} (y)}  \cdot \leq \lprp{C \ell \log \dmax}^{(i_{j - 1} - i_j) / 2} \cdot \wt{R}
        \end{gather*}
        with probability at least $1  - \delta / 8l$.
    \end{claim}
    \begin{proof}
        We start by constructing an $\eps$-net \cite[Definition 4.2.1]{vershynin}, $\mc{G}$, of $f_{i_j} (\mb{B} (x, R))$ with $\eps = \epsnetres$. Note that we may assume $\abs{\mc{G}} \leq (10 \wt{R} / \eps)^{d_{i_j}}$. We will prove the statement on the grid and extend to rest of the space. For layer $i + 1$, defining $\wt{x} = f_{i_j} (x)$, we have $\forall \wt{y} \in \mc{G}$:
        \begin{align*}
            \norm{\wt{f}_{i + 1, i_j} (\wt{x}) - \wt{f}_{i + 1, i_j} (\wt{y})} &= \norm{W_{i + 1} (f_{i, i_j}(\wt{x}) - f_{i, i_j}(\wt{y}))} \leq \norm{f_{i, i_j}(\wt{x}) - f_{i, i_j}(\wt{y})} \cdot \sqrt{\frac{d_{i + 1}}{d_i}} \cdot \lprp{1 + \sqrt{\frac{\log 1 / \delta^\prime}{d_{i + 1}}}}
        \end{align*}
        with probability at least $1 - \delta^\prime$ as before by \cref{thm:tsirelson}. By setting $\delta^\prime = \delta / (16 \abs{\mc{G}} \ell^2)$ and noting that $d_i \geq d_{i_j}$, the conclusion holds for layer $i + 1 \leq i_j$ on $\mc{G}$ with probability at least $1 - \delta / (16\ell^2)$. By induction and the union bound, we get:
        \begin{gather*}
            \forall i \in \{i_j + 1, \dots , i_{j - 1} - 1\}, \wt{y} \in \mc{G}: \norm{\wt{f}_{i, i_j} (\wt{y}) - \wt{f}_{i, i_j}(\wt{x})} \leq (C \ell \log \dmax)^{(i - i_j) / 2} \cdot \sqrt{\frac{d_i}{d_{i_j}}} \cdot \wt{R} \\
            \forall \wt{y} \in \mc{G}: \norm{\wt{f}_{i_{j - 1}, i_j} (\wt{y}) - \wt{f}_{i_{j - 1}, i_j}(\wt{x})} \leq \lprp{C \ell \log \dmax}^{(i_{j - 1} - i_j) / 2} \cdot \wt{R}
        \end{gather*}
        with probability at least $1 - \delta / (16\ell^2)$. To extend to all $y \in f_{i_j} (\B (x, R))$, we condition on \cref{lem:gau_spec_conc} for all $W_i$ with $i \leq i_{j - 1}$ and note that $\forall y \in f_{i_j} (\B (x, R))$, for $\wt{y} = \argmin_{z \in \mc{G}} \norm{z - y}$, and for $i_j+1\le i<i_{j-1}$,
        \begin{align*}
            \norm{\wt{f}_{i, i_j} (\wt{x}) - \wt{f}_{i, i_j} (y)} &\leq \norm{\wt{f}_{i, i_j} (\wt{x}) - \wt{f}_{i, i_j} (\wt{y})} + \norm{\wt{f}_{i, i_j} (y) - \wt{f}_{i, i_j} (\wt{y})} \\
            &\leq \norm{\wt{f}_{i, i_j} (\wt{x}) - \wt{f}_{i, i_j}
            (\wt{y})} + \norm{y - \wt{y}} \prod_{k = i_{j} + 1}^i
            \norm{W_k} \\
            &\leq \norm{\wt{f}_{i, i_j} (\wt{x}) - \wt{f}_{i, i_j}
            (\wt{y})} + \eps \prod_{k = i_{j} + 1}^i
            \left(C\sqrt{\frac{d_k}{d_{k-1}}}\right) \\
            &= \norm{\wt{f}_{i, i_j} (\wt{x}) - \wt{f}_{i, i_j}
            (\wt{y})} + \eps C^{i-i_j}
            \sqrt{\frac{d_i}{d_{i_j}}},
        \end{align*}
        using that $d_i\ge d_{i_j}$.
        Similarly, for $i=i_{j-1}$, we have
        \begin{align*}
            \norm{\wt{f}_{i_{j-1}, i_j} (\wt{x}) - \wt{f}_{i_{j-1}, i_j} (y)}
            &\leq \norm{\wt{f}_{i_{j-1}, i_j} (\wt{x}) -
            \wt{f}_{i_{j-1}, i_j}
            (\wt{y})} + \eps C^{i_{j-1}-i_j}
            \sqrt{\frac{d_{i_{j-1}-1}}{d_{i_j}}}.
        \end{align*}
        Our setting of $\eps$ concludes the proof of the claim.
\qed

==> content/checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes
  \item Did you describe the limitations of your work?
    \answerYes
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Our work is a theoretical exploration of an empirical phenomenon and we do not foresee it leading to any negative societal impacts.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes
	\item Did you include complete proofs of all theoretical results?
    \answerYes
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
  \answerNA
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
  \answerNA
  \item Did you mention the license of the assets?
  \answerNA
  \item Did you include any new assets either in the supplemental material or as a URL?
  \answerNA
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
  \answerNA
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
  \answerNA
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
  \answerNA
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
  \answerNA
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
  \answerNA
\end{enumerate}

\end{enumerate}


==> content/notes.tex <==
\section{Notes and ToDo}
\label{sec:notes}

% The proof will follow along the following lines:

% \begin{enumerate}
%     \item First show that the gradient is large at fixed $x$ (Easy) - Done
%     \item Show that the scale of the data remains roughly the same as it traverses through the layers in the model - Done
%     \begin{enumerate}
%         \item Show that the scale of $x$ remains roughly $\sqrt{d_i}$ at each layer - Done
%         \item Show that the other points remain in a bounded ball around $x$ (This will take a union bound over a net around $x$) - Done
%     \end{enumerate}
%     \item Use the gradient decomposition you thought about previously to finish the proof
%     \begin{enumerate}
%         \item Show that the spectral norm of prefixes of network segments remains bounded - Done
%         \item Imitate proof for previous point to show that each term in the gradient decomposition within a segment is vanishing - Done (Up to steps from previous proof)
%     \end{enumerate}
% \end{enumerate}

TODO:

\begin{enumerate}
    \item Write lemma for distributional equivalence
\end{enumerate}

==> content/relu_proof.tex <==
\section{Proof of Main Theorem}
\label{sec:proof_relu}

%We start by introducing some notation used throughout. We will use $d$ to
%denote the input dimension of the network, $\ell$ the number of layers
%and $d_1, \dots, d_\ell$ the dimensions of the intermediate layers of
%the network. The neural network has independent random weight
%matrices $W_i\in\mb{R}^{d_i\times d_{i-1}}$ for $i\in[\ell+1]$, where
%we set $d_0=d$ and $d_{\ell+1}=1$. Its output is defined as
%follows:
%
%\begin{gather}
%    f(x) = W_{\ell + 1}\cdot \sigma (W_{\ell}\cdot \sigma (W_{\ell -
%    1}\cdot \sigma ( \cdots \sigma (W_1\cdot x) \cdots ))) \text{ where } \sigma (x) = \max \{x, 0\} \text{ pointwise} \notag \\
%    W_{\ell + 1} \sim \mc{N} (0, I / d_\ell) \text{ and } (W_i)_{k, l}
%    \overset{i.i.d}{\thicksim} \mc{N} (0, 1 / d_{i-1}) \label{eq:nn_def} \tag{NN-DEF}.
%\end{gather}

\subsection{Concentration of Function Value and Gradient at a Fixed Point}
\label{sec:f_grad_anticonc}

Before we proceed, we introduce some additional notation used throughout the proof. For $x \in \mb{R}^d$, we let:
\begin{equation*}
    x_0 \coloneqq x, 
    \quad \wt{f}_i (x) \coloneqq W_i f_{i - 1} (x),
    \quad (D_{i} (y))_{j,k} = 
    \begin{cases}
        0 & \text{if } j \neq k \\
        \bm{1} \{y_j \geq 0\} & \text{otherwise}
    \end{cases},
    \quad x_i = D_i (\wt{f}_i (x)) \wt{f}_i (x). \tag{FIX-NOT}
\end{equation*}
Hence, $f(x) = \wt{f}_{\ell + 1} (x)$.

\begin{lemma}
    \label{lem:f_grad_conc}
    % For any $\norm{x} = \sqrt{d}$,
    For some universal constant $c$ and any $\norm{x} = \sqrt{d}$,
    with probability at least $1 - \delta$ we have:
    \begin{equation*}
        % \left|f(x)\right| \leq 2^{\ell + 3} \sqrt{\log 1 / \delta}
        \left|f(x)\right| \leq c2^{\ell} \sqrt{\log 1 / \delta}
        \text{ and } \norm{\nabla f(x)} \geq \frac{1}{2^{\ell +
        1}},
    \end{equation*}
    provided $\min_{0\le i\le\ell}d_i\ge c(1+\ln(\ell/\delta))$.
\end{lemma}
\begin{proof}
    Note that
    \begin{equation*}
        \nabla f (x) = W_{\ell + 1} \prod_{i = \ell}^1 D_i (\wt{f}_i (x)) W_i \text{ and } f(x) = \nabla f (x) x.
    \end{equation*}
    From the spherical symmetry of the Gaussian distribution,
    \begin{equation*}
        \nabla f(x) \overset{d}{=} \tilde{W}_{\ell + 1} \prod_{i = \ell}^1 D_i \tilde{W}_i \text{ where } 
        (D_i)_{j,k} = \begin{cases}
                        0 & \text{if }  j \neq k \\
                        1 & \text{with probability } 1/2 \\
                        0 & \text{with probability } 1/2
                      \end{cases}
        \text{ and } \{W_i\}_{i = 1}^{\ell + 1} \overset{d}{=}
        \{\tilde{W}_i\}_{i = 1}^{\ell + 1}.
    \end{equation*}
    Therefore, it suffices to analyze the random vector
    $\tilde{W}_{\ell + 1} \prod_{i = \ell}^1 D_i \tilde{W}_i$. We
    first condition on a favorable event for the $D_i$. Note that we
    have by the union bound and an application of Hoeffding's
    inequality (e.g.,~\cite[Theorem 2.8]{blm})
    that:
    \begin{equation*}
        \forall i \in [\ell]: \Tr D_i \geq \frac{d_i}{3} \text{ with probability at least } 1 - \delta / 4,
    \end{equation*}
    provided $d_i\ge c\log(4/\delta)$. We now condition on the $D_i$ and note that:
    \begin{gather*}
        \norm*{\wt{W}_{\ell + 1} \prod_{i = \ell}^1 D_i \wt{W}_i} \overset{d}{=} \norm*{W^\dagger_{\ell + 1} \prod_{i = \ell}^1 W^\dagger_{i}} \text{ where } \\
        \forall i \in \{2, \dots, \ell\}: W^\dagger_i \in \R^{\Tr D_i \times \Tr D_{i - 1}},\ W^\dagger_{\ell + 1} \in \R^{1 \times \Tr D_\ell},\ W^\dagger_{1} \in \R^{\Tr D_1 \times d} \\
        (W^\dagger_1)_{j, :} \thicksim \mc{N} (0, I / d),\
        W^\dagger_{\ell + 1} \thicksim \mc{N} (0, I / d_\ell),\
        \forall i \in \{2, \dots, \ell + 1\}: (W^\dagger_i)_{j, :}
        \thicksim \mc{N} \lprp{0, I/d_{i - 1}}.
    \end{gather*}
    From the above display, we obtain from \cref{thm:tsirelson}
    applied to $f(x) = -\norm{x}$:
    \begin{align*}
        \norm*{W^\dagger_{\ell + 1} \prod_{i = \ell}^1 W^\dagger_i} &\geq \frac{1}{2} \cdot \norm*{W^\dagger_{\ell + 1} \prod_{i = \ell}^2 W^\dagger_i} && \text{with probability at least } 1 - \delta / (4\ell) \\
        &\geq \frac{1}{2^{\ell + 1}} && \text{with probability at least } 1 - \delta / 4 \text{ by induction},
    \end{align*}
    provided $\min_{0\le i\le\ell} d_i\ge c\log(4\ell/\delta)$.
    Through a similar argument, we obtain:
    \begin{equation}
        \label{eq:grad_ub}
        \norm*{\tilde{W}_{\ell + 1} \prod_{i = \ell}^1 D_i \tilde{W}_i} \leq 2^{\ell + 1}
    \end{equation}
    with probability at least $1 - \delta / 4$. We also have:
    \begin{gather*}
        \lprp{\tilde{W}_{\ell + 1} \prod_{i = \ell}^1 D_i \tilde{W}_i
        \; \Biggr |\; \norm*{\tilde{W}_{\ell + 1} \prod_{i = \ell}^1
        D_i \tilde{W}_i} = m} \overset{d}{=} \mrm{Unif} \lprp{m
        \mb{S}^{d - 1}}.
        % \forall v \in \mb{R}^d, q,t \in \mb{R}_+: \mb{P}_{x \sim \mrm{Unif} (q \mb{S}^{d - 1})} \lbrb{\abs{\inp{v}{x}} \geq t} \leq 2 \mb{P}_{x \sim \mc{N} (0, 2 m I / d)} \lbrb{\abs{\inp{v}{x}} \geq t}.
    \end{gather*}
    Combining this, \cref{eq:grad_ub,lem:gau_unif_comp}, we get that:
    \begin{equation*}
        %\left|f(x)\right| \leq 2^{\ell + 3} \sqrt{\log 1 / \delta}
        \left|f(x)\right| \leq c2^{\ell} \sqrt{\log 1 / \delta}
    \end{equation*}
    with probability at least $1 - \delta / 2$,
    for some absolute constant $c$.
    A union bound over all the preceeding events concludes the lemma.
\end{proof}

\subsection{Scale Preservation of Local Neighborhoods}
\label{ssec:scale_pres_local_nbrhood}

In this section, we show that the image of a ball around $x$ remains in a ball of suitable radius around the image of $x$ projected through the various layers of the network. This is made formal in \cref{lem:scale_pres_ml}.
% Our first lemma is a simple concentration inequality on the $\norm{W_i}$.
%
% \begin{lemma}
%     \label{lem:w_spec_conc}
%     We have:
%     \begin{equation*}
%         \norm{W_i} \leq C \lprp{1 + \sqrt{\frac{d_i}{d_{i - 1}}} + \sqrt{\frac{\log 1 / \delta}{d_{i - 1}}}}
%     \end{equation*}
%     with probability at least $1 - \delta$.
% \end{lemma}
% \begin{proof}
%     The proof follows from \cref{lem:gau_spec_conc}.
% \end{proof}
We will use the following notation in the proof. We
use $m_i$ to denote the bottleneck layer for layer $i$ and $\dmini$ to
denote its width. We also introduce notation for intermediate
vector-valued functions computed by the network, both from an input
to a layer and from one layer to a later one.
\begin{gather*}
    \dmax = \max_{i \in [\ell]} d_i, \quad \dmini = \min_{j < i} d_j, \quad \mini = \argmin_{j < i} d_j\\ 
    f_0(x) = x, \quad \wt{f}_i (x) = W_i f_{i - 1} (x), 
    \quad (D_{i} (y))_{j,k} = 
    \begin{cases}
        0 & \text{if } j \neq k \\
        \bm{1} \{y_j \geq 0\} & \text{otherwise}
    \end{cases},
    \quad f_i (x) = D_i (\wt{f}_i (x)) \wt{f}_i (x) \\
    \forall j \in \{0\} \cup [\ell + 1]: f_{j, j} (x) = x, \quad  \forall i > j: \wt{f}_{i, j} (x) = W_i f_{i-1, j} (x), \quad f_{i, j} (x) = D_i(\wt{f}_{i , j}(x)) \wt{f}_{i, j} (x)\tag{SP-NOT} \label{eq:sp_not}
\end{gather*}

In the subsequent lemma and its proof, we will decompose the network
into different segments and analyze its behavior in each of these
segments separately. This decomposition is crucial for reducing
the sizes of the $\epsilon$-nets that arise in the discretization
arguments in our proofs. The segments will be defined by indices
$\lbrb{i_j}_{j = 1}^m$, which represent a sequence of bottleneck
layers, defined recursively from the output layer backwards:
\begin{equation*}
    i_1 \coloneqq \argmin_{i \leq \ell} d_i, \qquad \forall j > 1
    \text{ s.t } i_j > 1,\, i_{j + 1} \coloneqq \argmin_{j < i_j} d_j \tag{NN-DECOMP} \label{eq:nn_dec}.
\end{equation*}
We will refer to the segment of the network from the output of layer
$i_{j+1}$ to the output of layer $i_j$ as the $j$th segment of the
network.

\begin{lemma}
    \label{lem:scale_pres_ml}
    We have for any $R \leq \dmax$,
    \begin{gather*}
        \forall i \in [\ell]: \norm{f_i(x)} \geq \lprp{\frac{1}{2}}^i \cdot \sqrt{d_i}\\
        \forall \norm{x' - x} \leq R: \norm{\wt{f}_i (x) - \wt{f}_i (x')} \leq \lprp{C \log \dmax}^{i / 2} \cdot \lprp{1 + \sqrt{\frac{d_i}{\dmini}}} \cdot R \\
        \forall \norm{x' - x} \leq R: \norm{f_i (x) - f_i (x')} \leq \lprp{C \log \dmax}^{i / 2} \cdot \lprp{1 + \sqrt{\frac{d_i}{\dmini}}} \cdot R
    \end{gather*}
    for a suitably large constant $C > 0$ with probability at least $1 - \delta$.
\end{lemma}
\begin{proof}
    We start with the first claim of the lemma. As in the proof of \cref{lem:f_grad_conc}, we note that:
    \begin{gather*}
        f_i (x) = \prod_{j = i}^1 D_i(\wt{f}_i (x)) W_i x\\
        \norm*{\prod_{j = i}^1 D_i(\wt{f}_i (x)) W_i} \overset{d}{=} \norm*{\prod_{j = i}^1 D_i \wt{W}_i} \text{ where } 
        (D_i)_{j,k} = \begin{cases}
            0 & \text{if }  j \neq k \\
            1 & \text{with probability } 1/2 \\
            0 & \text{with probability } 1/2
          \end{cases}
\text{ and } \{W_i\}_{i = 1}^{\ell + 1} \overset{d}{=} \{\wt{W}_i\}_{i = 1}^{\ell + 1}.
    \end{gather*}
    Therefore, it suffices to analyze the distribution of $\prod_{j = i}^1 D_j \wt{W}_j x$. Again, we condition on the following event:
    \begin{equation*}
        \forall i \in [\ell]: \Tr D_i \geq \frac{d_i}{3}
    \end{equation*}
    which occurs with probability at least $1 - \delta / 8$. As in the proof of \cref{lem:f_grad_conc}, we observe the following distributional equivalence:
    \begin{gather*}
        \forall i \in [\ell]: \norm*{\prod_{j = i}^1 D_j \wt{W}_j (x)} \overset{d}{=} \norm*{\prod_{j = i}^1 W^\dagger_j x} \text{ where } \forall j \in \{2, \dots, i\} \in W^\dagger_j \in \R^{\Tr D_j \times \Tr D_{j - 1}},\ W^\dagger_1 \in \R^{\Tr D_1 \times d} \\
        \forall j \in \{2, \dots, i\} (W^\dagger_j)_{k, :} \thicksim \mc{N} \lprp{0, I / d_{j - 1}}, (W^\dagger_1)_{k, :} \thicksim \mc{N} (0, I / d).
    \end{gather*}
    A recursive application of \cref{thm:tsirelson} as in the proof of \cref{lem:f_grad_conc} yields:
    \begin{equation*}
        \norm*{\prod_{j = i}^1 D_j \wt{W}_j x} \geq \lprp{\frac{1}{2}}^i
    \end{equation*}
    with probability at least $1 - \delta / 16\ell^2$. A union bound over the $j$ layers concludes the proof of the first claim of the lemma.
    % \begin{align*}
    %     \norm*{\prod_{j = i}^1 D_j \wt{W}_j x} &\geq \frac{1}{2} \cdot \sqrt{\frac{d_i}{d_{i - 1}}}\norm*{\prod_{j = i - 1}^1 D_j \wt{W}_j x} && \text{Conditioning on } \prod_{j = i - 1}^1 D_j \wt{W}_j x \\ &\geq \lprp{\frac{1}{2}}^i \sqrt{d_i} && \text{By induction with probability at least } 1 - \delta / (8\ell).
    % \end{align*}
    % A union bound over the $j$ layers concludes the proof of the first claim of the lemma.

    % We will establish the second claim through a gridding based argument with some subtleties. Namely, we construct a new grid over the image of $\mb{B}(x,R)$ whenever the number of units in a hidden layer drops. With this outline in mind, we start by splitting our neural network into a series of segments. We define these segments inductively as follows:
    % \begin{equation*}
    %     i_1 = \ell, \qquad i_{j + 1} \coloneqq \argmin_{j < i_j} d_j
    % \end{equation*}
    % with segments implicitly defined by indices $\{i_j\}_{j = 1}^m$. Note $m \leq \ell$ and for $i_{j + 1} < i < i_j$, we have $d_i \geq d_{i_{j + 1}}$. We now establish the following claim inductively:
    We will establish the second claim through a gridding based argument with some subtleties. Namely, we construct a new grid over the image of $\mb{B}(x,R)$ whenever the number of units in a hidden layer drops lower than all the previous layers in the network starting from the input layer. These layers are precisely defined by the indices $i_j$ in \ref{eq:nn_dec}. We now establish the following claim inductively.
    \begin{claim}
        \label{clm:per_segmend_sp}
        Suppose for $j > 1$ and $\wt{R} \leq \dmax \cdot R$:
        \begin{equation*}
            \forall y \in \mb{B} (x, R): \norm{f_{i_j}(x) - f_{i_j} (y)} \leq \wt{R}.
        \end{equation*}
        Then:
        \begin{gather*}
            \forall i \in \{i_j + 1, \dots, i_{j - 1} - 1\}, y \in
            \mb{B} (x, R): \norm{\wt{f}_i (x) - \wt{f}_i (y)} \leq \lprp{C \ell \log
            \dmax}^{(i - i_j) / 2} \cdot \sqrt{\frac{d_i}{d_{i_j}}}
            \cdot \wt{R}, \\
            \forall y \in \mb{B} (x, R): \norm{\wt{f}_{i_{j-1}} (x) -
            \wt{f}_{i_{j-1}} (y)}  \cdot \leq \lprp{C \ell \log \dmax}^{(i_{j - 1} - i_j) / 2} \cdot \wt{R}
        \end{gather*}
        with probability at least $1  - \delta / 8l$.
    \end{claim}
    \begin{proof}
        We start by constructing an $\eps$-net \cite[Definition 4.2.1]{vershynin}, $\mc{G}$, of $f_{i_j} (\mb{B} (x, R))$ with $\eps = \epsnetres$. Note that we may assume $\abs{\mc{G}} \leq (10 \wt{R} / \eps)^{d_{i_j}}$. We will prove the statement on the grid and extend to rest of the space. For layer $i + 1$, defining $\wt{x} = f_{i_j} (x)$, we have $\forall \wt{y} \in \mc{G}$:
        \begin{align*}
            \norm{\wt{f}_{i + 1, i_j} (\wt{x}) - \wt{f}_{i + 1, i_j} (\wt{y})} &= \norm{W_{i + 1} (f_{i, i_j}(\wt{x}) - f_{i, i_j}(\wt{y}))} \leq \norm{f_{i, i_j}(\wt{x}) - f_{i, i_j}(\wt{y})} \cdot \sqrt{\frac{d_{i + 1}}{d_i}} \cdot \lprp{1 + \sqrt{\frac{\log 1 / \delta^\prime}{d_{i + 1}}}}
        \end{align*}
        with probability at least $1 - \delta^\prime$ as before by \cref{thm:tsirelson}. By setting $\delta^\prime = \delta / (16 \abs{\mc{G}} \ell^2)$ and noting that $d_i \geq d_{i_j}$, the conclusion holds for layer $i + 1 \leq i_j$ on $\mc{G}$ with probability at least $1 - \delta / (16\ell^2)$. By induction and the union bound, we get:
        \begin{gather*}
            \forall i \in \{i_j + 1, \dots , i_{j - 1} - 1\}, \wt{y} \in \mc{G}: \norm{\wt{f}_{i, i_j} (\wt{y}) - \wt{f}_{i, i_j}(\wt{x})} \leq (C \ell \log \dmax)^{(i - i_j) / 2} \cdot \sqrt{\frac{d_i}{d_{i_j}}} \cdot \wt{R} \\
            \forall \wt{y} \in \mc{G}: \norm{\wt{f}_{i_{j - 1}, i_j} (\wt{y}) - \wt{f}_{i_{j - 1}, i_j}(\wt{x})} \leq \lprp{C \ell \log \dmax}^{(i_{j - 1} - i_j) / 2} \cdot \wt{R}
        \end{gather*}
        with probability at least $1 - \delta / (16\ell^2)$. To extend to all $y \in f_{i_j} (\B (x, R))$, we condition on \cref{lem:gau_spec_conc} for all $W_i$ with $i \leq i_{j - 1}$ and note that $\forall y \in f_{i_j} (\B (x, R))$, for $\wt{y} = \argmin_{z \in \mc{G}} \norm{z - y}$, and for $i_j+1\le i<i_{j-1}$,
        \begin{align*}
            \norm{\wt{f}_{i, i_j} (\wt{x}) - \wt{f}_{i, i_j} (y)} &\leq \norm{\wt{f}_{i, i_j} (\wt{x}) - \wt{f}_{i, i_j} (\wt{y})} + \norm{\wt{f}_{i, i_j} (y) - \wt{f}_{i, i_j} (\wt{y})} \\
            &\leq \norm{\wt{f}_{i, i_j} (\wt{x}) - \wt{f}_{i, i_j}
            (\wt{y})} + \norm{y - \wt{y}} \prod_{k = i_{j} + 1}^i
            \norm{W_k} \\
            &\leq \norm{\wt{f}_{i, i_j} (\wt{x}) - \wt{f}_{i, i_j}
            (\wt{y})} + \eps \prod_{k = i_{j} + 1}^i
            \left(C\sqrt{\frac{d_k}{d_{k-1}}}\right) \\
            &= \norm{\wt{f}_{i, i_j} (\wt{x}) - \wt{f}_{i, i_j}
            (\wt{y})} + \eps C^{i-i_j}
            \sqrt{\frac{d_i}{d_{i_j}}},
        \end{align*}
        using that $d_i\ge d_{i_j}$.
        Similarly, for $i=i_{j-1}$, we have
        \begin{align*}
            \norm{\wt{f}_{i_{j-1}, i_j} (\wt{x}) - \wt{f}_{i_{j-1}, i_j} (y)}
            &\leq \norm{\wt{f}_{i_{j-1}, i_j} (\wt{x}) -
            \wt{f}_{i_{j-1}, i_j}
            (\wt{y})} + \eps C^{i_{j-1}-i_j}
            \sqrt{\frac{d_{i_{j-1}-1}}{d_{i_j}}}.
        \end{align*}
        Our setting of $\eps$ concludes the proof of the claim.
    \end{proof}

    An inductive application of \cref{clm:per_segmend_sp}, a union bound and the observation that:
    \begin{equation*}
        \norm{f_i (x) - f_i (y)} \leq \norm{\wt{f}_i (x) - \wt{f}_i (y)}
    \end{equation*}
    concludes the proof of the lemma.
\end{proof}

\begin{lemma}
    \label{lem:x_i_anticonc}
    For all $i \in [\ell]$, we have:
    \begin{equation*}
        \#\lbrb{j: \abs{\inp{(W_{i + 1})_j}{x_i}} \geq \alpha_i
        \frac{\norm{x_i}}{\sqrt{d_i}}} \geq \lprp{1 -
        2\sqrt{\frac{2}{\pi}}\alpha_i} d_{i + 1}
    \end{equation*}
    with probability at least $1 - \delta$, provided
    $d_{i+1}\alpha_i^2\ge \ln(l/\delta)$.
\end{lemma}
\begin{proof}
    Follows from the fact that $\Pr(|Z|\le c)\le c\sqrt{2/\pi}$ for
    $Z\sim N(0,1)$, plus a simple application of Heoffding's Inequality.
\end{proof}

\subsection{Proving Local Gradient Smoothness}
\label{ssec:local_grad_smooth}

In this section, we show that the gradient is locally smooth which will imply the existence of adversarial examples. Adopting notation from \ref{eq:nn_def} and \ref{eq:sp_not}, we observe the following gradient decomposition:
\begin{align*}
    &\nabla f(x) - \nabla f(y) \\
    &= W_{\ell + 1} \prod_{i = \ell}^1 D_i(\wt{f}_i(x)) W_i - W_{\ell + 1} \prod_{i = \ell}^1 D_i(\wt{f}_i(y)) W_i = W_{\ell + 1} \lprp{\prod_{i = \ell}^1 D_i(\wt{f}_i(x)) W_i - \prod_{i = \ell}^1 D_i(\wt{f}_i(y)) W_i} \\
    &= W_{\ell + 1} \lprp{\prod_{i = \ell}^1 D_i(\wt{f}_i(x)) W_i - (D_\ell (\wt{f}_\ell (x)) + (D_\ell (\wt{f}_\ell (y)) - D_\ell (\wt{f}_\ell (x)))) W_\ell\prod_{i = \ell - 1}^1 D_i(\wt{f}_i(y)) W_i} \\
    &= W_{\ell + 1} \lprp{D_\ell (\wt{f}_\ell (x)) W_\ell \lprp{\prod_{i = \ell - 1}^1 D_i(\wt{f}_i(x)) W_i - \prod_{i = \ell - 1}^1 D_i(\wt{f}_i(y))W_i} + (D_\ell (\wt{f}_\ell (x)) - D_\ell (\wt{f}_\ell (y))) W_\ell \prod_{i = \ell - 1}^1 D_i(\wt{f}_i(y)) W_i} \\
    &= \sum_{j = 1}^\ell W_{\ell + 1} \lprp{\prod_{i = \ell}^{j + 1} D_i(\wt{f}_i(x)) W_i}\cdot (D_j(\wt{f}_j (x)) - D_j(\wt{f}_j (y))) W_j \cdot \lprp{\prod_{k = j - 1}^1 D_i(\wt{f}_i(y)) W_i} \tag{GD-DECOMP} \label{eq:grad_decomp}.
\end{align*}

Therefore, it suffices to bound each of the terms in expansion. Before
we proceed, we prove a structural lemma on the spectral norm of the
matrices appearing in the right-hand-side of the final expression in
\ref{eq:grad_decomp}. This will use the partitioning of the network as
in \cref{lem:scale_pres_ml} where the first layer in each segment is
the narrowest. We introduce some notation: for $i>j$, define
\begin{equation*}
    M_{i, j} (y) = \prod_{k = i}^{j + 1} D_k (\wt{f}_k(y)) W_k
\end{equation*}
and state and prove the lemma below:
\begin{lemma}
    \label{lem:nn_part_spec_bnd}
    We have:
    \begin{equation*}
        \forall \norm{y - x} \leq R, j \in [m]: \norm*{M_{i_j, i_{j + 1}} (y)} \leq (C \cdot \ell \cdot \log \dmax)^{(i_j - i_{j + 1}) / 2}
    \end{equation*}
    with probability at least $1 - \delta$.
\end{lemma}
\begin{proof}
    To start, consider a fixed $j \in [m]$ and condition on the conclusion of \cref{lem:scale_pres_ml} upto level $i_{j + 1}$. Now, consider an $\eps$-net of $f_{i_{j + 1}} (\mb{B} (x, R))$, $\mc{G}$, with resolution $\eps = \epsnetres$. As before, $\abs{\mc{G}} \leq (\dmax)^{48\ell d_{i_{j + 1}}}$ for some constant $C$. We additionally will consider subsets
    \begin{equation*}
        \mc{S} = \lbrb{(S_k)_{k = i_j - 1}^{i_{j + 1} + 1}:
        S_k\subseteq[d_k],\, \abs{S_k} \leq 4 d_{i_{j + 1}}}.
    \end{equation*}
    Note that $\abs{\mc{G}} \cdot \abs{\mc{S}}^2 \leq (\dmax)^{64ld_{i_{j + 1}}}$. For $y \in \mc{G}, S^1, S^2 \in \mc{S}$, consider the following matrix:
    \begin{equation*}
        M^{i_{j}, i_{j + 1}}_{y, S^1, S^2} = \prod_{k = i_{j}}^{i_{j + 1} + 1} (D_k (\wt{f}_{k, i_j} (y))) + (D_{S^1_k} - D_{S^2_k})) W_k \text{ where } 
        (D_S)_{i, j} = 
        \begin{cases}
            1, \text{if } i = j \text{ and } i \in S \\
            0, \text{otherwise}
        \end{cases}.
    \end{equation*}
    We will bound the spectral norm of $M^{i_{j}, i_{j + 1}}_{y, S^1, S^2}$. First, note that:
    \begin{equation*}
        \norm*{M^{i_j, i_{j + 1}}_{y, S^1, S^2}} \leq \norm*{\wt{M}^{i_j, i_{j + 1}}_{y, S^1, S^2}} \text{ where } \wt{M}^{i_j, i_{j + 1}}_{y, S^1, S^2} \coloneqq W_{i_j} \prod_{k = i_{j} - 1}^{i_{j + 1} + 1} (D_k (\wt{f}_{k, i_j} (y)) + (D_{S^1_k} - D_{S^2_k})) W_k
    \end{equation*}
    and observe that:
    \begin{equation*}
        \wt{M}^{i_{j}, i_{j + 1}}_{y, S^1, S^2} \overset{d}{=} W_{i_j} \prod_{k = i_{j} - 1}^{i_{j + 1} + 1} (D_k + (D_{S^1_k} - D_{S^2_k})) W_k) \text{ where }
        (D_k)_{i,j} = 
        \begin{cases}
            1, \text{with probability } \frac{1}{2} \text{ if } i = j\\
            0, \text{otherwise}
        \end{cases}.
    \end{equation*}
    To bound the spectral norm, let $\mc{B}$ be a $1/3$-net of $\S^{d_{i_j} - 1}$ and $v \in \mc{B}$:
    \begin{align*}
        \norm*{v^\top \wt{M}^{i_j, i_{j + 1}}_{y, S^1, S^2}} &\leq \norm*{v^\top W_{i_j} \prod_{k = i_j - 1}^{i_{j + 1} + 2} (D_k +  (D_{S^1_k} - D_{S^2_k})) W_k)} \cdot \lprp{1 + \sqrt{\frac{\log 1 / \delta^\prime}{d_{i_{j + 1}}}}} \leq \prod_{k = i_{j}}^{i_{j + 1}} \lprp{1 + \sqrt{\frac{\log 1 / \delta^\prime}{d_{k}}}}
    \end{align*}
    with probability at least $\ell \delta^\prime$. But setting $\delta^\prime = \delta / (16 \ell^4 \cdot \abs{\mc{G}} \cdot \abs{\mc{S}} \cdot \abs{\mc{B}})$ yields with probability at least $1 - \delta /16$:
    \begin{equation*}
        \forall y \in \mc{G}, S_1, S_2 \in \mc{S}:
         \norm{W_{i_j}} \cdot (C \cdot \ell \cdot \log \dmax)^{(i_j - i_{j + 1}) / 2}.
    \end{equation*}
    For $y \notin \mc{G}$, the following claim concludes the proof of the lemma:
    \begin{claim}
        \label{clm:grid_approx_act_patt_spec_bnd}
        We have:
        \begin{equation*}
            \forall m \in \{i_{j - 1}, \dots, i_j\}, y \in f_{i_j} (\mb{B} (x, R)): \Tr \abs{D_m (\wt{f}_{m, i_j} (y)) - D_m (\wt{f}_{m, i_j} (\wt{y}))} \leq 4d_{i_j} \text{ where } \wt{y} = \argmin_{z \in \mc{G}} \norm{z - y}
        \end{equation*}
        with probability at least $1 - \delta^\prime / \ell^2$.
    \end{claim}
    \begin{proof}
        We start by conditioning on the conclusion of \cref{lem:gau_spec_conc} upto layer $i_{j - 1}$. Then:
        \begin{equation*}
            \forall m \in \{i_{j - 1}, \cdots, i_j\}, y \in f_{i_j} (\mb{B} (x, R)): \norm{\wt{f}_{m, i_{j}} (y) - \wt{f}_{m, i_j} (\wt{y})} \leq \eps \cdot \lprp{C \dmax}^{(m - i_j) / 2}.
        \end{equation*}
        Now, let $m \in \{i_{j - 1}, \cdots, i_j + 1\}$ and $y \in \mc{G}$. We have:
        \begin{multline*}
            \max_{z \text{ s.t } \norm{z - y} \leq \eps} \# \{i: \sign (\inp{(W_m)_{i, :}}{f_{m - 1, i_j} (y)}) \neq \sign (\inp{(W_m)_{i, :}}{f_{m - 1, i_j}} (z))\} \\
            \leq \# \{i: \exists z \text{ s.t } \norm{z - y} \leq \eps \text{ and } \sign (\inp{(W_m)_{i, :}}{f_{m - 1, i_j} (y)}) \neq \sign (\inp{(W_m)_{i, :}}{f_{m - 1, i_j} (z)})\}.
        \end{multline*}
        Defining
        \begin{equation*}
            W_i(y) \coloneqq \bm{1} \{\exists z \text{ s.t } \norm{z - y} \leq \eps \text{ and } \sign (\inp{(W_m)_{i, :}}{f_{m - 1, i_j} (y)}) \neq \sign (\inp{(W_m)_{i, :}}{f_{m - 1, i_j} (z)})\},
        \end{equation*}
        we get:
        \begin{align*}
            \P \lbrb{W_i(y) = 1} &\leq \P  \lbrb{(C \dmax)^{(m - i_j) / 2} \cdot \eps \cdot \norm{w_i} \geq \abs{\inp{w_i}{y}}} \\
            &\leq \P \lbrb{\norm{w_i} \geq 2} + \P \lbrb{2\eps (C \dmax)^{(m - i_j) / 2} \geq \abs{\inp{w_i}{y}}} \leq \eps \cdot (C \dmax)^{(m - i_j) / 2}.
        \end{align*}
        Therefore, we have:
        \begin{equation*}
            \P \lbrb{\sum_{i = 1}^{d_m} W_i(y) \geq 4d_{i_k}} \leq d_m^{4d_{i_j}} \cdot \lprp{\eps (C \dmax)^{(m - i_k) / 2}}^{4d_{i_j}}
        \end{equation*}
        and hence by the union bound and our setting of $\eps$ and bound on $\mc{G}$:
        \begin{equation*}
            \P \lbrb{\exists y \in \mc{G}: \sum_{i = 1}^{d_m} W_i (y) \geq 4d_{i_j}} \leq (C\dmax)^{60 \ell d_{i_j}} \cdot \eps^{4 d_{i_j}} \leq \frac{\delta'}{16\ell^4}.
        \end{equation*}
    \end{proof}
\end{proof}

We proceed to do so in the following lemma:
\begin{lemma}
    \label{lem:ind_error_bnd}
    We have:
    \begin{equation*}
        \forall \norm{x - y} \leq R, j \in [\ell]: \norm{\nabla f(x) - \nabla f(y)} \leq \frac{1}{\log^\ell \dmax}
    \end{equation*}
    with probability at least $1 - \delta$.
\end{lemma}
\begin{proof}
    Consider a fixed term in the decomposition of the gradient difference from \ref{eq:grad_decomp}; that is, consider the random vector-valued function:
    \begin{equation*}
        \gddiff_j(y) \coloneqq W_{\ell + 1} \lprp{\prod_{i = \ell}^{j + 1} D_i(\wt{f}_i(x)) W_i} \cdot (D_j(\wt{f}_j (y)) - D_j(\wt{f}_j (x))) W_j \cdot \lprp{\prod_{k = j - 1}^1 D_i(\wt{f}_i(y)) W_i}.
    \end{equation*}
    We will show with high probability that $\gddiff_j(y) = o(1)$ with high probability for all $\norm{x - y} \leq R$. This will then imply the lemma by an union bound and \ref{eq:grad_decomp}. Let $k$ be such that $i_k = \argmin_{m < j} d_m$. We will condition on the weights of the network up to layer $i_k$. Specifically, we will assume the conclusions of \cref{lem:scale_pres_ml,lem:nn_part_spec_bnd} up to layer $i_k$. We may now focus our attention solely on the segment of the network beyond layer $i_k$ as a consequence of the following observations:
    \begin{multline*}
        \norm*{\gddiff_j(y)} \\
        \leq \norm*{W_{\ell + 1} \lprp{\prod_{i = \ell}^{j + 1} D_i(\wt{f}_i(x)) W_i} \cdot (D_j(\wt{f}_j (y)) - D_j(\wt{f}_j (x))) W_j \cdot \lprp{\prod_{k = j - 1}^{i_k} D_i(\wt{f}_i(y)) W_i}} \cdot \norm*{\prod_{k = i_k}^1 D_i(\wt{f}_i(y)) W_i}
    \end{multline*}
    
    Observe now that:
    \begin{gather*}
        W_{\ell + 1} \prod_{j = \ell}^{j + 1} D_i(\wt{f}_i(x)) W_i \overset{d}{=} \wt{W}_{\ell + 1} \prod_{j = \ell}^{j + 1} D_i \wt{W}_i \eqqcolon H \text{ where } \\
        (D_i)_{m, n} = 
        \begin{cases}
            1, &\text{with probability } 1/2 \text{ if } m = n \\
            0, &\text{otherwise}
        \end{cases},
        \{W_i\}_{i = j + 1}^{\ell + 1} \overset{d}{=} \{\wt{W}_i\}_{i = j + 1}^{\ell + 1}
    \end{gather*}
    Therefore, $H$ is a spherically-symmetric random vector and we condition on the following high probability bound on its length:
    \begin{align}
        \label{eq:h_l_bnd_gd_proof}
        \norm{H} &\leq \norm*{\wt{W}_{\ell + 1} \prod_{j = \ell}^{j + 2} D_i \wt{W}_i} \cdot \lprp{1 + 2\sqrt{\frac{\log \ell / \delta^\prime}{d_j}}} \leq \lprp{2}^{\ell + 1 - j}
    \end{align}
    with probability at least $1 - \delta^\prime$ and setting $\delta^\prime = \delta / (64\ell^2)$. Observe that the distribution of $H$ remains spherically symmetric even after conditioning on the above event. As in the proof of \cref{lem:nn_part_spec_bnd}, let $\mc{G}$ be an $\eps$-net of $f_{i_k}(\mb{B} (x, R))$ with $\eps$ as in the proof of \cref{lem:nn_part_spec_bnd}. We now show a basic structural claim of how activations pattern differ across the various layers between a point and its closest approximation in $\mc{G}$:
    \begin{claim}
        \label{clm:grid_approx_act_patt}
        We have:
        \begin{equation*}
            \forall m \in \{i_{k - 1}, \dots, i_k\}, y \in f_{i_k} (\mb{B} (x, R)): \Tr \abs{D_m (\wt{f}_{m, i_k} (y)) - D_m (\wt{f}_{m, i_k} (\wt{y}))} \leq 4d_{i_k} \text{ where } \wt{y} = \argmin_{z \in \mc{G}} \norm{z - y}
        \end{equation*}
        with probability at least $1 - \delta^\prime / \ell^2$.
    \end{claim}
    \begin{proof}
        The proof is identical to the proof of \cref{clm:grid_approx_act_patt_spec_bnd}.
        % We start by conditioning on the conclusion of \cref{lem:gau_spec_conc} upto layer $i_{k - 1}$. Then:
        % \begin{equation*}
        %     \forall m \in \{i_{k - 1}, \cdots, i_k\}, y \in f_{i_k} (\mb{B} (x, R)): \norm{\wt{f}_{m, i_{k}} (y) - \wt{f}_{m, i+k} (\wt{y})} \leq \eps \cdot \lprp{C \dmax}^{(m - i_k) / 2}.
        % \end{equation*}
        % Now, let $m \in \{i_{k - 1}, \cdots, i_k + 1\}$ and $y \in \mc{G}$. We have:
        % \begin{multline*}
        %     \max_{z \text{ s.t } \norm{z - y} \leq \eps} \# \{i: \sign ((W_m)_i^\top f_{m - 1, i_k} (y)) \neq \sign ((W_m)_i^\top f_{m - 1, i_k} (z))\} \\
        %     \leq \# \{i: \exists z \text{ s.t } \norm{z - y} \leq \eps \text{ and } \sign ((W_m)_i^\top f_{m - 1, i_k} (y)) \neq \sign ((W_m)_i^\top f_{m - 1, i_k} (z))\}.
        % \end{multline*}
        % Defining
        % \begin{equation*}
        %     W_i(y) \coloneqq \bm{1} \{\exists z \text{ s.t } \norm{z - y} \leq \eps \text{ and } \sign ((W_m)_i^\top f_{m - 1, i_k} (y)) \neq \sign ((W_m)_i^\top f_{m - 1, i_k} (z))\},
        % \end{equation*}
        % we get:
        % \begin{align*}
        %     \P \lbrb{W_i(y) = 1} &\leq \P  \lbrb{(C \dmax)^{(m - i_k) / 2} \cdot \eps \cdot \norm{w_i} \geq \abs{\inp{w_i}{y}}} \\
        %     &\leq \P \lbrb{\norm{w_i} \geq 2} + \P \lbrb{2\eps (C \dmax)^{(m - i_k) / 2} \geq \abs{\inp{w_i}{y}}} \leq \eps \cdot (C \dmax)^{(m - i_k) / 2}.
        % \end{align*}
        % Therefore, we have:
        % \begin{equation*}
        %     \P \lbrb{\sum_{i = 1}^{d_m} W_i(y) \geq 4d_{i_k}} \leq d_m^{4d_{i_k}} \cdot \lprp{\eps (C \dmax)^{(m - i_k) / 2}}^{4d_{i_k}}
        % \end{equation*}
        % and hence by the union bound:
        % \begin{equation*}
        %     \P \lbrb{\exists y \in \mc{G}: \sum_{i = 1}^{d_m} W_i (y) \geq 4d_{i_k}} \leq (C\dmax)^{4 \ell d_{i_k}} \cdot \eps^{4 d_{i_k}} \leq \frac{\delta'}{16\ell^4}.
        % \end{equation*}
    \end{proof}
    
    
    We now break into two cases depending on how $d_{j}$ compares to $d_{i_k}$ and handle them separately.
    
    \paragraph{Case 1:} $d_j \leq d_{i_k} (\ell \log^{\ell} \dmax)^{20}$. In this case, define the sets $\mc{S}, \mc{Q}$ as follows:
    \begin{equation*}
        \mc{S} \coloneqq \lbrb{(S_m)_{m = i_k + 1}^{j - 1}: S_m \subseteq [d_m],\ \abs{S_m} \leq 4\cdot d_{i_k}},\qquad \mc{Q} \coloneqq \lbrb{Q: Q \subset [d_j],\ \abs{Q} \leq \frac{d_j}{(\ell \log \dmax)^{60\ell}}}.
    \end{equation*}
    Now, for $Q^1, Q^2 \subset \mc{Q}, y \in \mc{G}, S^1, S^2 \in \mc{S}$, define the random vector:
    \begin{equation*}
        V^{j, k}_{y, Q^1, Q^2, S^1, S^2} = H (D_{Q^1} - D_{Q^2}) W_j \prod_{m = j - 1}^{i_k + 1} (D_m (\wt{f}_{m, i_k} (y)) + (D_{S^1_m} - D_{S^2_m})) W_m.
    \end{equation*}
    Note that:
    \begin{equation*}
        V^{j, k}_{y, Q^1, Q^2, S^1, S^2} \overset{d}{=} H (D_{Q^1} - D_{Q^2}) W_j \prod_{m = j - 1}^{i_k + 1} (D_m + (D_{S^1_m} - D_{S^2_m})) W_m \text{ where } 
        (D_m)_{i,j} = 
        \begin{cases}
            1, &\text{w.p } 1/2 \text{ if } i = j\\
            0, &\text{otherwise}
        \end{cases}.
    \end{equation*}
    Note that $\abs{\mc{Q}}^2 \cdot \abs{\mc{G}} \cdot \abs{\abs{S}}^2 \leq (\dmax)^{64 \ell d_{i_k}}$. We now get:
    \begin{align*}
        \norm*{V^{j, k}_{y, Q^1, Q^2, S_1, S_2}} &\leq \norm*{H (D_{Q^1} - D_{Q^2}) W_j \prod_{m = j - 1}^{i_k + 2} (D_m + (D_{S^1_m} - D_{S^2_m})) W_m} \cdot \lprp{1 + \sqrt{\frac{\log 1 / \delta^\dagger}{d_{i_k}}}} \\
        &\leq \norm{H (D_{Q^1} - D_{Q^2})} \cdot \prod_{m = i_k + 1}^{j} \lprp{1 + \sqrt{\frac{\log 1 / \delta^\dagger}{d_{m - 1}}}} \\
        &\leq \norm{H (D_{Q^1} - D_{Q^2})} \cdot (C \ell \log \dmax)^{(j - i_k) / 2}
    \end{align*}
    where the final inequality follows from the fact that $d_m \geq d_{i_k}$ and by setting $\delta^\dagger = \delta / (32 \cdot \ell^4 \cdot \abs{\mc{Q}}^2 \cdot \abs{\mc{G}} \cdot \abs{\mc{S}}^2)$. A union bound now implies that the previous conclusion holds for all $Q^1, Q^2 \in \mc{Q}, y \in \mc{G}, S^1, S^2 \in \mc{S}$. For the first term, we use the trivial bound:
    \begin{equation*}
        \norm{H (D_{Q^1} - D_{Q^2})} \leq \sqrt{\abs{Q^1} + \abs{Q^2}} \cdot \max_m \abs{H_m} \leq 10 \cdot \sqrt{\frac{d_j}{(\ell \log \dmax)^{60\ell}}} \cdot  \sqrt{\frac{\norm{H}^2}{d_j} \cdot (\log \dmax + \log \ell / \delta)}.
    \end{equation*}
    with probability at least $1 - \delta / (32 \cdot \ell^4)$ from \cref{lem:gau_unif_comp}. 
    
    To conclude the proof, we get from \cref{lem:x_i_anticonc,lem:scale_pres_ml}, for all $y \text{ s.t } \norm{y - x} \leq R$:
    \begin{align*}
        &\Tr \abs{D_j (\wt{f}_j (y)) - D_j (\wt{f}_j (y))} \\
        &\leq \#\lbrb{i: \abs{\inp{f_{j - 1} (x)}{(W_j)_i}} \leq \frac{\norm{f_{j - 1} (x)}}{4 \sqrt{d_{j - 1}} \cdot (\ell \log \dmax)^{75 \ell}}} + \frac{\norm{\wt{f}_j (x) - \wt{f}_j (y)}^2}{\norm{f_{j - 1} (x)}^2}\cdot 16 \cdot d_{j - 1} \cdot \lprp{\ell \log \dmax}^{150\ell}\\
        &\leq \frac{d_j}{2 (\ell \log \dmax)^{75 \ell}} + d_j \cdot \lprp{\frac{R^2}{\dmin}}\cdot \frac{(C \ell \log \dmax)^{\ell}}{d_{j - 1}} \cdot 16 \cdot d_{j - 1} \cdot \lprp{\ell \log \dmax}^{150\ell} \leq \frac{d_j}{(\ell \log \dmax)^{60\ell}}.
    \end{align*}
    Hence, we get with probability at least $1 - \delta / (16 \ell^4)$:
    \begin{gather*}
        \forall \norm{y - x} \leq R : \Tr \abs{D_j (\wt{f}_j (y)) - D_j (\wt{f}_j (x))} \leq \frac{d_j}{(\ell \log \dmax)^{60\ell}}, \\
        \forall \norm{y - x} \leq R, \forall m \in \{i_k + 1, \dots, j - 1\}: \Tr \abs{D_m (\wt{f}_{m} (y)) - D_m (\wt{f}_{m, i_k} (\wt{y}))} \leq 4d
    \end{gather*}
    where $\wt{y} = \argmin_{z \in \mc{G}} \norm{z - f_{i_k} (y)}$. Our bound from \cref{eq:h_l_bnd_gd_proof} now concludes the proof in this case.

    \paragraph{Case 2:} $d_j \geq d_{i_k} (\ell \log^{\ell} \dmax)^{20}$. As in the previous case, we start by defining the sets $\mc{S}$:
    \begin{equation*}
        \mc{S} = \lbrb{(S_m)_{m = i_k + 1}^{j - 1}: S_m \subseteq [d_m],\ \abs{S_m} \leq 4\cdot d_{i_k}}.
    \end{equation*}
    Now, for $y \in \mc{G}, S^1, S^2 \in \mc{S}$, consider the random matrix:
    \begin{gather*}
        M^{j, k}_{y, S^1, S^2} \coloneqq W_{j - 1} \prod_{m = j - 2}^{i_k + 1} (D_m (\wt{f}_m (y)) + (D_{S_m^1} - D_{S_m^2})) W_m \\
        M^{j, k}_{y, S^1, S^2} \overset{d}{=} \wt{W}_{j - 1} \prod_{m = j - 2}^{i_k + 1} (D_m + (D_{S_m^1} - D_{S_m^2})) \wt{W}_m.
    \end{gather*}
    We will bound the spectral norm of $M^{j,k}_{y, S^1, S^2}$ for all $y,S^1,S^2$ with high probability as follows. Let $\mc{V}$ be a $1/9$-grid of $\mb{S}^{d_{i_k}}$ and $v \in \mc{V}$. We have:
    \begin{align}
        \norm*{M^{j, k}_{y, S^1, S^2}v} &\leq \sqrt{\frac{d_{j - 1}}{d_{j - 2}}} \cdot \lprp{1 + \sqrt{\frac{\log 1 / \delta^\dagger}{d_{j - 1}}}} \cdot \norm*{\prod_{m = j - 2}^{i_k + 1} (D_m + (D_{S_m^1} - D_{S_m^2})) \wt{W}_m v} \notag \\
        &\leq \sqrt{\frac{d_{j - 1}}{d_{i_k}}} \cdot \prod_{m = i_k + 1}^{j - 1} \lprp{1 + \sqrt{\frac{\log 1 / \delta^\dagger}{d_m}}} \leq \sqrt{\frac{d_{j - 1}}{d_{i_k}}} \cdot \lprp{C \ell \log \dmax}^{(j - i_k + 1) / 2} \label{eq:jk_spec_bnd}
    \end{align}
    where the final inequality follows by the fact that $d_m \geq d_{i_k}$ and by setting $\delta^\dagger = \delta / (32 \cdot \ell \cdot \abs{\mc{G}} \cdot \abs{\mc{S}}^2 \cdot \mc{V})$. By a union bound, the bound on the spectral norms of $M^{j,k}_{y, S^1, S^2}$ follows. We now condition on this event and the conclusion of \cref{lem:scale_pres_ml} up to layer $j - 1$ for the rest of the proof. 

    Let $\wt{M}^{j,k}_{y, S^1, S^2} = D_{j - 1}(\wt{f}_{j - 1, i_k} (y)) \cdot M^{j,k}_{y, S^1, S^2}$ and for $y \in \mc{G}$, let $\wt{y} = f_{j - 1, i_k} (y)$ and $\wt{x} = f_{j - 1} (x)$. We have by an application of \cref{lem:large_width_proof_gd_diff_bnd} and a union bound over all $y \in \mc{G}, S^1, S^2 \in \mc{S}$:
    \begin{equation*}
        \forall y \in \mc{G}, S^1, S^2 \in \mc{S}: \norm*{H^\top (D_{j} (\wt{f}_{j, i_k} (y)) - D_j (\wt{f}_{j} (x))) \wt{M}^{j,k}_{y, S^1, S^2}} \leq \lprp{\frac{C}{\ell \log \dmax}}^{3\ell}
    \end{equation*}
    with probability at least $1 - \delta'/\ell^2$.
    
    % We obtain:
    % \begin{multline*}
    %     \norm*{H (D_j(\wt{y}) - D_j (\wt{y})) W_j \wt{M}^{j, k}_{y, S^1, S^2, b}} \\
    %     \leq \norm*{H (D_j(\wt{y}) - D_j (\wt{y})) W_j \mc{P}_V \wt{M}^{j, k}_{y, S^1, S^2, b}} + \norm*{H (D_j(\wt{y}) - D_j (\wt{y})) W_j \mc{P}_V^\perp \wt{M}^{j, k}_{y, S^1, S^2, b}}
    % \end{multline*}
    % Each of the two terms in the above expression is at most $1 / \poly \log^\ell \dmax$ from first analysis in the one layer case\ynote{Formalize this fully. Use spherical symmetry in the orthogonal setting and small scale when in $V$}. 
    
    To conclude the proof, we additionally condition on $\norm{H}_\infty$. We have as a consequence of \cref{lem:gau_unif_comp} that:
    \begin{equation*}
        \norm{H}_\infty \leq 4 \cdot 2^{\ell + 1 - j} \cdot \sqrt{\frac{\log d_j + \log 1 / \delta^\dagger}{d_j}}
    \end{equation*}
    with probability at least $1 - \delta^\dagger$. We condition on this event and proceed as follows. Let $T \subset [d_j]$ such that $\abs{T} \leq 4 \cdot d_{i_k}$ and $y \in \mc{G}, S^1, S^2, \in \mc{S}$ and we observe:
    \begin{equation*}
        \norm*{H^\top D_T \wt{W}_j \wt{M}^{j, k}_{y, S^1, S^2}} \leq \norm*{H^\top D_T \wt{W}_j U^{j,k}_{y, S^1, S^2}} \cdot \norm*{\wt{M}^{j, k}_{y, S^1, S^2}}
    \end{equation*}
    where $U^{j,k}_{y, S^1, S^2}$ are the left singular vectors of $\wt{M}^{j,k}_{y, S^1, S^2}$ and observe:
    \begin{align*}
        \P \lbrb{\norm*{H^\top D_T \wt{W}_j U^{j,k}_{y, S^1, S^2}} \geq t} = \P_{\wt{Z} \thicksim \mc{N} \lprp{0, \norm{H D_T}^2 \cdot \frac{I}{d_j}}} \lbrb{\norm{\wt{Z}} \geq t} \leq \P_{Z \thicksim \mc{N} \lprp{0, \norm{H}_\infty^2 \cdot \abs{T} \cdot \frac{I}{d_j}}} \lbrb{\norm{Z} \geq t}
    \end{align*}
    to get that (conditioned on $H$ and noting that $\mrm{rank} (U^{j,k}_{y, S^1, S^2}) \leq d_{i_k}$):
    \begin{equation*}
        \norm*{H^\top D_T U^{j,k}_{y, S^1, S^2}} \leq \norm{H}_\infty \cdot \sqrt{\abs{T}} \cdot \sqrt{\frac{d_{i_k}}{d_j}} \cdot \lprp{1 + \sqrt{\frac{\log 1 / \delta^\ddagger}{d_{i_k}}}}
    \end{equation*}
    By setting $\delta^\ddagger = \delta / (128 \ell^2 d_j^{4d_{i_k}} \abs{\mc{S}}^2 \abs{\mc{G}})$ and our bounds on $d_j, T$ yield:
    \begin{equation*}
        \forall T \subset [d_j] \text{ s.t } \abs{T} \leq 4d_{i_k}, y \in \mc{G}, S^1, S^2 \in \mc{S}: \norm*{H^\top D_T U^{j,k}_{y, S^1, S^2}} \leq \frac{1}{(\ell \log \dmax)^{4\ell}}
    \end{equation*}
    with probability at least $1 - \delta / (64 \ell^2)$. Along with \cref{clm:grid_approx_act_patt} and \cref{eq:jk_spec_bnd}, this concludes the proof in this case.

    A union bound over all $j \in [\ell]$ and a triangle inequality with \ref{eq:grad_decomp} yields the final statement in the lemma.
\end{proof}

\begin{lemma}
    \label{lem:large_width_proof_gd_diff_bnd}
    Let $L, R, r > 0, k,m,n \in \mb{N}, M \in \mb{R}^{m \times n}$ such that $m \geq n$. Furthermore, suppose $W \in \mb{R}^{k \times m}$ and $H$ is distributed as follows:
    \begin{equation*}  
        W = 
        \begin{bmatrix}
            w_1^\top \\
            w_2^\top \\
            \vdots \\
            w_k^\top
        \end{bmatrix}
        \text{ with }
        w_i \overset{i.i.d}{\thicksim} \mc{N} (0, I / m), 
        \text{ and } H \thicksim \mathrm{Unif} (L\cdot \mb{S}^{k - 1}).
    \end{equation*}
    Furthermore, suppose $x \in \mb{R}^m$ satisfies $\norm{x} \geq R$ and $y$ be such that $\norm{y - x} \leq r$. Then:
    \begin{gather*}
        \mb{P} \lbrb{\norm{H^\top D W M} \geq 1024 \cdot \norm{M} \cdot L \cdot \lprp{\sqrt{\frac{r}{R} \log 2R/r \cdot \lprp{\frac{n + \log 1 / \delta^\dagger}{m}}} + \lprp{\frac{n + \log 1 / \delta^\dagger}{\sqrt{km}}}}} \leq \delta^\dagger \\
        \text{ where } D_{i,j} = 
        \begin{cases}
            0, & \text{if } i \neq j \\
            \bm{1} \lbrb{w_i^\top x \geq 0} - \bm{1} \lbrb{w_i^\top y \geq 0}, & \text{otherwise}
        \end{cases}.
    \end{gather*}
\end{lemma}
\begin{proof}
    Note that it suffices to analyze the random variable:
    \begin{equation*}
        \wt{H}^\top D W M \text{ for } \wt{H} \thicksim \mc{N} (0, 2L^2 \cdot I / k).
    \end{equation*}
    Let $V$ denote the two-dimensional subspace of $\mb{R}^m$ containing $x,y$. We now decompose the norm as follows:
    \begin{equation}
        \label{eq:diff_decomp}
        \norm{\wt{H}^\top D W M} \leq \norm{\wt{H}^\top D W \proj_V M} + \norm{\wt{H}^\top D W \proj_V^\perp M} \leq \norm{\wt{H}^\top D W \proj_V}\cdot \norm{M} + \norm{\wt{H}^\top D W \proj_V^\perp M}.
    \end{equation}
    To apply Bernstein's inequality, we first expand on the first term:
    \begin{align*}
        \wt{H}^\top D W \proj_V = \sum_{i = 1}^k \wt{H}_i D_{i,i} \proj_V w_i.
    \end{align*}
    Letting $Z_i = \wt{H}_i D_{i,i} \proj_V w_i$, we note that $\E [Z_i] = 0$ and bound its even moments as follows:
    \begin{align*}
        \E \lsrs{\inp{v_j}{Z_i}^2} &= \E \lsrs{\wt{H}_i^2 \cdot D_{i,i}^2 \cdot \inp{v_j}{w_i}^2} \leq \frac{2L^2}{k} \cdot \E \lsrs{\norm{\proj_V w_i}^2} \cdot \P \lbrb{D_{i,i} \neq 0} = \frac{2L^2}{k} \cdot \frac{2}{m} \cdot \P \lbrb{D_{i,i} \neq 0} \\
        \E \lsrs{\inp{v_j}{Z_i}^\ell} &= \E \lsrs{\wt{H}_i^\ell \cdot D_{i,i}^\ell \cdot \inp{v_j}{w_i}^\ell} \leq (\ell - 1)!! \lprp{\frac{2L^2}{k}}^{\ell / 2} \cdot \E \lsrs{\norm{\proj_V w_i}^\ell} \cdot \P \lbrb{D_{i,i} \neq 0} \\
        &\leq (\ell - 1)!! \lprp{\frac{2L^2}{k}}^{\ell / 2} \cdot \lprp{2^{\ell / 2} \cdot \E \lsrs{\inp{w_i}{v_1}^\ell + \inp{w_i}{v_2}^\ell}} \cdot \P \lbrb{D_{i,i} \neq 0} \\
        &= 2\cdot (\ell - 1)!! \lprp{\frac{4L^2}{k}}^{\ell / 2} \cdot \E \lsrs{\inp{w_i}{v_1}^\ell} \cdot \P \lbrb{D_{i,i} \neq 0} = 2 \cdot ((\ell - 1)!!)^{2} \lprp{\frac{4L^2}{km}}^{\ell / 2} \cdot \P \lbrb{D_{i,i} \neq 0} \\
        &\leq 2 \cdot \ell! \cdot \lprp{\frac{8L^2}{km}}^{\ell / 2} \cdot \P \lbrb{D_{i,i} \neq 0}.
    \end{align*}
    For odd $\ell \geq 3$ we have by a similar manipulations:
    \begin{align*}
        \E \lsrs{\abs{\inp{v_j}{Z_i}}^\ell} &= \E \lsrs{\abs*{\wt{H}_i^\ell \cdot D_{i,i}^\ell \cdot \inp{v_j}{w_i}^\ell}} \leq \P \lbrb{D_{i,i} \neq 0} \cdot \E \lsrs{\abs{\wt{H}_i^\ell \cdot \norm{\proj_V w_i}^\ell}} \\
        &\leq \P \lbrb{D_{i,i} \neq 0} \cdot \sqrt{\E \lsrs{\lprp{\wt{H}_i \cdot \norm{\proj_V w_i}}^{2\ell}}} \leq \P \lbrb{D_{i,i} \neq 0} \cdot \sqrt{2 \cdot (2\ell)! \cdot \lprp{\frac{8L^2}{km}}^{\ell}} \\
        &\leq \P \lbrb{D_{i,i} \neq 0} \cdot \sqrt{2 \cdot (2\ell)!} \cdot \lprp{\frac{8L^2}{km}}^{\ell / 2} \leq \P \lbrb{D_{i,i} \neq 0} \cdot 2^\ell \ell! \cdot \lprp{\frac{8L^2}{km}}^{\ell / 2} \\
        &\leq \P \lbrb{D_{i,i} \neq 0} \cdot \ell! \cdot \lprp{\frac{32L^2}{km}}^{\ell / 2}
    \end{align*}
    By a union bound and an application of \cref{thm:bernstein} gives:
    \begin{equation*}
        \norm*{\sum_{i = 1}^k Z_i} \leq 2\max_{j \in \{1,2\}} \abs*{\sum_{i = 1}^k \inp{v_j}{Z_i}} \leq 256 \cdot L \cdot \lprp{\sqrt{\frac{1}{m} \cdot \P \lbrb{D_{i,i} \neq 0} \cdot \log 1 / \delta'} + \frac{\log 1 / \delta'}{\sqrt{km}}}
    \end{equation*}
    with probability at least $1 - \delta'$ via a union bound. 

    For the other term in \cref{eq:diff_decomp}, we use $U$ to denote the left singular subspace of $M$ and $Y$ to denote the span of the left singular vectors of $\proj_V^\perp \proj_U$ with non-zero singular values. Noting $\norm{\proj_V^\perp \proj_U} \leq 1$, we now have:
    \begin{equation*}
        \norm{\wt{H}^\top D W \proj_V^\perp M} \leq \norm{M} \cdot \norm{\wt{H}^\top D W \proj_V^\perp \proj_U} \leq \norm{M} \cdot \norm{\wt{H}^\top DW \proj_Y}.
    \end{equation*}
    We expand the term on the right as follows:
    \begin{equation*}
        \wt{H}^\top D W \proj_Y = \sum_{i = 1}^k \wt{H}_i D_{i,i} \proj_Y w_i = \sum_{i = 1}^k D_{i,i} \cdot \lprp{\wt{H}_i \proj_Y w_i} \eqqcolon Y_i.
    \end{equation*}
    Note that $Y$ is orthogonal to $V$ as $\proj_V (\proj_V^\perp \proj_U u) = 0$ for all $u$ and hence, $\wt{H}_i \proj_Y w_i$ and $D_{i,i}$ are independent random variables (due to $\proj_V w_i$ and $\proj_V^\perp w_i$ being independent). Now, let $y \in Y \text{ s.t }\norm{y} = 1$ and we bound the directional even moments of $Y_i$ with the aim of applying Bernstein's inequality as before:
    \begin{align*}
        \E \lsrs{\inp{y}{Y_i}^2} &= \E \lsrs{D_{i,i}^2 \cdot \wt{H}_i^2 \cdot \inp{y}{w_i}^2} = \frac{2L^2}{k} \cdot \frac{1}{m} \cdot \P \lbrb{D_{i,i} \neq 0} \\
        \E \lsrs{\inp{y}{Y_i}^\ell} &= \E \lsrs{D_{i,i}^\ell \cdot \wt{H}_i^\ell \cdot \inp{y}{w_i}^\ell} = \lprp{(\ell - 1)!!}^2 \cdot \lprp{\frac{2L^2}{km}}^{\ell / 2} \cdot \P \lbrb {D_{i,i} \neq 0} \leq \ell! \cdot \lprp{\frac{2L^2}{km}}^{\ell / 2} \cdot \P \lbrb{D_{i,i} \neq 0}.
    \end{align*}
    Similarly, for odd $\ell \geq 3$, we have:
    For odd $\ell \geq 3$ we have by a similar manipulations:
    \begin{align*}
        \E \lsrs{\abs{\inp{y}{Y_i}}^\ell} &= \E \lsrs{\abs*{\wt{H}_i^\ell \cdot D_{i,i}^\ell \cdot \inp{y}{w_i}^\ell}} \leq \P \lbrb{D_{i,i} \neq 0} \cdot \E \lsrs{\abs{\wt{H}_i^\ell \cdot \inp{y}{w_i}^\ell}} \\
        &\leq \P \lbrb{D_{i,i} \neq 0} \cdot \sqrt{\E \lsrs{\abs{\wt{H}_i^\ell \cdot \inp{y}{w_i}^{2\ell}}}} \leq \P \lbrb{D_{i,i} \neq 0} \cdot \sqrt{(2\ell)! \cdot \lprp{\frac{2L^2}{km}}^{\ell}} \\
        &\leq \P \lbrb{D_{i,i} \neq 0} \cdot \sqrt{(2\ell)!} \cdot \lprp{\frac{2L^2}{km}}^{\ell / 2} \leq \P \lbrb{D_{i,i} \neq 0} \cdot 2^\ell \ell! \cdot \lprp{\frac{2L^2}{km}}^{\ell / 2} \\
        &\leq \P \lbrb{D_{i,i} \neq 0} \cdot \ell! \cdot \lprp{\frac{8L^2}{km}}^{\ell / 2}
    \end{align*}

    Now, consider a $1/3$-net of $\mc{G} \coloneqq Y \cap \S^{m - 1}$, $\wt{\mc{G}}$ and we get for any $z \in Y$ where $\wt{y} = \argmin_{z \in \mc{G}} \norm{y - z}$:
    \begin{equation*}
        \norm{z} = \max_{y \in \mc{G}} \inp{y}{z} = \max_{y \in \mc{G}} \inp{y - \wt{y}}{z} + \inp{\wt{y}}{z} \leq \max_{y \in \mc{\wt{G}}} \inp{y}{z} - \frac{\norm{z}}{3} \implies \norm{z} \leq \frac{3}{2} \max_{y \in \mc{G}} \inp{y}{z}.
    \end{equation*}
    Since the rank of $Y$ is at most $n$, We may assume $\abs{\mc{G}} \leq (30)^{n}$\cite[Corollary 4.2.13]{vershynin}. By a union bound:
    \begin{equation*}
        \norm*{\sum_{i = 1}^n Y_i} \leq 2 \max_{y \in \mc{\wt{G}}} \inp*{y}{\sum_{i = 1}^n Y_i} \leq 256 \cdot L \cdot \lprp{\sqrt{\P \lbrb{D_{i,i} \neq 0} \cdot \lprp{\frac{n + \log 1 / \delta'}{m}}} + \lprp{\frac{n + \log 1 / \delta'}{\sqrt{km}}}}
    \end{equation*}
    with probability at least $1 - \delta'$. The lemma follows from the previous discussion and \cref{lem:mis_sign_prob} by picking $\delta' = \delta^\dagger / 4$ and applying a union bound.
\end{proof}


==> content/relu_proof_old.tex <==
\section{Proof of Result for ReLU}
\label{sec:proof_relu}

We start by introducing some notation used throughout. We will use $d$ to
denote the input dimension of the network, $\ell$ the number of layers
and $d_1, \dots, d_\ell$ the dimensions of the intermediate layers of
the network. The neural network has independent random weight
matrices $W_i\in\mb{R}^{d_i\times d_{i-1}}$ for $i\in[\ell+1]$, where
we set $d_0=d$ and $d_{\ell+1}=1$. Its output is defined as
follows:

\begin{gather}
    f(x) = W_{\ell + 1}\cdot \sigma (W_{\ell}\cdot \sigma (W_{\ell -
    1}\cdot \sigma ( \cdots \sigma (W_1\cdot x) \cdots ))) \text{ where } \sigma (x) = \max \{x, 0\} \text{ pointwise} \notag \\
    W_{\ell + 1} \sim \mc{N} (0, I / d_\ell) \text{ and } (W_i)_{k, l}
    \overset{i.i.d}{\thicksim} \mc{N} (0, 1 / d_{i-1}) \label{eq:nn_def} \tag{NN-DEF}.
\end{gather}

\subsection{Fixed Point Function value and Gradient Concentration}
\label{sec:f_grad_anticonc}

Before we proceed, we introduce some additional notation used throughout the proof. For $x \in \mb{R}^d$, we let:
\begin{equation*}
    x_0 \coloneqq x, 
    \quad \tilde{x}_i \coloneqq W_i x_{i - 1},
    \quad (D_{i} (x))_{j,k} = 
    \begin{cases}
        0 & \text{if } j \neq k \\
        \bm{1} \{\tilde x_{ij} \geq 0\} & \text{otherwise}
    \end{cases},
    \quad x_i = D_i (x) \tilde x_i. \tag{FIX-NOT}
\end{equation*}
Hence, $f(x) = \tilde x_{\ell + 1}$.

\begin{lemma}
    \label{lem:f_grad_conc}
    For any $\norm{x} = \sqrt{d}$, we have:
    \begin{equation*}
        \left|f(x)\right| \leq 2^{\ell + 3} \sqrt{\log 1 / \delta} \leq \text{ and } \norm{\nabla f(x)} \geq \frac{1}{2^{\ell + 1}}
    \end{equation*}
    with probability at least $1 - \delta$.
\end{lemma}
\begin{proof}
    Note that we have:
    \begin{equation*}
        \nabla f (x) = W_{\ell + 1} \prod_{i = \ell}^1 D_i (x) W_i \text{ and } f(x) = \nabla f (x) x.
    \end{equation*}
    We have from the spherical symmetry of the Gaussian distribution that:
    \begin{equation*}
        \nabla f(x) \overset{d}{=} \tilde{W}_{\ell + 1} \prod_{i = \ell}^1 D_i \tilde{W}_i \text{ where } 
        (D_i)_{j,k} = \begin{cases}
                        0 & \text{if }  j \neq k \\
                        1 & \text{with probability } 1/2 \\
                        0 & \text{with probability } 1/2
                      \end{cases}
        \text{ and } \{W_i\}_{i = 1}^{\ell + 1} \overset{d}{=}
        \{\tilde{W}_i\}_{i = 1}^{\ell + 1}.
    \end{equation*}
    Therefore, it suffices to analyze the random vector
    $\tilde{W}_{\ell + 1} \prod_{i = \ell}^1 D_i \tilde{W}_i$. We
    first condition on a favorable event for the $D_i$. Note that we
    have by the union bound and an application of Hoeffding's
    inequality (e.g.,~\cite[Theorem 2.8]{blm})
    that:
    \begin{equation*}
        \forall i \in [\ell]: \Tr D_i \geq \frac{d_i}{3} \text{ with probability at least } 1 - \delta / 4,
    \end{equation*}
    provided $d_i\ge c\ln(4/\delta)$. We now condition on the $D_i$ and note that:
    \begin{gather*}
        \norm*{\wt{W}_{\ell + 1} \prod_{i = \ell}^1 D_i \wt{W}_i} \overset{d}{=} \norm*{W^\dagger_{\ell + 1} \prod_{i = \ell}^1 W^\dagger_{i}} \text{ where } \\
        \forall i \in \{2, \dots, \ell\}: W^\dagger_i \in \R^{\Tr D_i \times \Tr D_{i - 1}},\ W^\dagger_{\ell + 1} \in \R^{1 \times \Tr D_\ell},\ W^\dagger_{1} \in \R^{\Tr D_1 \times d} \\
        \forall i \in \{2, \dots, \ell + 1\}: (W^\dagger_i)_{j, :} \thicksim \mc{N} \lprp{0, \frac{I}{d_{i - 1}}} \text{ and } (W^\dagger_1)_{j, :} \thicksim \mc{N} (0, I / d).
    \end{gather*}
    From the above display, we obtain from \cref{thm:tsirelson} applied to $f(x) = \norm{x}$:
    \begin{align*}
        \norm*{W^\dagger_{\ell + 1} \prod_{i = \ell}^1 W^\dagger_i} &\geq \frac{1}{2} \cdot \norm*{W^\dagger_{\ell + 1} \prod_{i = \ell}^2 W^\dagger_i} && \text{with probability at least } 1 - \delta / (4\ell) \\
        &\geq \frac{1}{2^{\ell + 1}} && \text{with probability at least } 1 - \delta / 4 \text{ by induction}.
    \end{align*}
    Through a similar argument, we obtain:
    \begin{equation}
        \label{eq:grad_ub}
        \norm*{\tilde{W}_{\ell + 1} \prod_{i = \ell}^1 D_i \tilde{W}_i} \leq 2^{\ell + 1}
    \end{equation}
    with probability at least $1 - \delta / 4$. We now have the following facts:
    \begin{gather*}
        \lprp{\tilde{W}_{\ell + 1} \prod_{i = \ell}^1 D_i \tilde{W}_i \; \Biggr |\; \norm*{\tilde{W}_{\ell + 1} \prod_{i = \ell}^1 D_i \tilde{W}_i} = m} \overset{d}{=} \mrm{Unif} \lprp{m \mb{S}^{d - 1}} \\
        \forall v \in \mb{R}^d, q,t \in \mb{R}_+: \mb{P}_{x \sim \mrm{Unif} (q \mb{S}^{d - 1})} \lbrb{\abs{\inp{v}{x}} \geq t} \leq 2 \mb{P}_{x \sim \mc{N} (0, 2 m I / d)} \lbrb{\abs{\inp{v}{x}} \geq t}.
    \end{gather*}
    From \cref{eq:grad_ub}, we get that:
    \begin{equation*}
        \left|f(x)\right| \leq 2^{\ell + 3} \sqrt{\log 1 / \delta}
    \end{equation*}
    with probability at least $1 - \delta / 2$. A union bound over all the preceeding events concludes the lemma.
\end{proof}

\subsection{Scale Preservation of Local Neighborhood}
\label{ssec:scale_pres_local_nbrhood}

Here, we show that the image of a ball around $x$ remains in a ball of suitable radius around the image of $x$ projected through the various layers of the network. This is made formal in \cref{lem:scale_pres_ml}. Our first lemma is a simple concentration inequality on the $\norm{W_i}$.

\begin{lemma}
    \label{lem:w_spec_conc}
    We have:
    \begin{equation*}
        \norm{W_i} \leq C \lprp{1 + \sqrt{\frac{d_i}{d_{i - 1}}} + \sqrt{\frac{\log 1 / \delta}{d_{i - 1}}}}
    \end{equation*}
    with probability at least $1 - \delta$.
\end{lemma}
\begin{proof}
    The proof follows from \cref{lem:gau_spec_conc}.
\end{proof}

We will use the following notation in the proof of the main lemma of this subsection:
\begin{gather*}
    \dmax = \max_{i \in [\ell]} d_i, \quad \dmini = \min_{j < i} d_j, \quad \mini = \argmin_{j < i} d_j\\ 
    f_0(x) = x, \quad \wt{f}_i (x) = W_i f_{i - 1} (x), 
    \quad (D_{i} (y))_{j,k} = 
    \begin{cases}
        0 & \text{if } j \neq k \\
        \bm{1} \{y_j \geq 0\} & \text{otherwise}
    \end{cases},
    \quad f_i (x) = D_i (\wt{f}_i (x)) \wt{f}_i (x) \\
    \forall j \in \{0\} \cup [\ell + 1]: f_{j, j} (x) = x, \quad  \forall i > j: \wt{f}_{i, j} (x) = W_i f_{i-1, j} (x), \quad f_{i, j} (x) = D_i(\wt{f}_{i , j}(x)) \wt{f}_{i, j} (x)\tag{SP-NOT} \label{eq:sp_not}
\end{gather*}

In the subsequent lemma and its proof, we will decompose the network into different segments and analyze its behavior in each of these segments separately. Our gridding arguments will crucially require this decomposition to reduce the sizes of the grids arising in our proofs. The segments will be defined by indices $\lbrb{i_j}_{j = 1}^m$ defined recursively below:
\begin{equation*}
    i_1 \coloneqq \ell, \qquad \forall j > 1 \text{ s.t } i_j > 1: i_{j + 1} \coloneqq \argmin_{j < i_j} d_j \tag{NN-DECOMP} \label{eq:nn_dec}.
\end{equation*}
We will analyze the behavior of the network from the output of layer $i_j$ to the output of layer $i_{j - 1}$. 

\begin{lemma}
    \label{lem:scale_pres_ml}
    We have for any $R \leq \poly (\dmax)$
    \begin{gather*}
        \forall i \in [\ell]: \norm{f_i(x)} \geq \lprp{\frac{1}{2}}^i \cdot \sqrt{d_i}\\
        \forall \norm{x' - x} \leq R: \norm{\wt{f}_i (x) - \wt{f}_i (x')} \leq \lprp{C \log \dmax}^{i / 2} \cdot \lprp{1 + \sqrt{\frac{d_i}{\dmini}}} \cdot R \\
        \forall \norm{x' - x} \leq R: \norm{f_i (x) - f_i (x')} \leq \lprp{C \log \dmax}^{i / 2} \cdot \lprp{1 + \sqrt{\frac{d_i}{\dmini}}} \cdot R
    \end{gather*}
    with probability at least $1 - \delta$.
\end{lemma}
\begin{proof}
    We start with the first claim of the lemma. As in the proof of \cref{lem:f_grad_conc}, we note that:
    \begin{gather*}
        f_i (x) = \prod_{j = i}^1 D_i(x) W_i x\\
        \prod_{j = i}^1 D_i(x) W_i \overset{d}{=} \prod_{j = i}^1 D_i \wt{W}_i \text{ where } 
        (D_i)_{j,k} = \begin{cases}
            0 & \text{if }  j \neq k \\
            1 & \text{with probability } 1/2 \\
            0 & \text{with probability } 1/2
          \end{cases}
\text{ and } \{W_i\}_{i = 1}^{\ell + 1} \overset{d}{=} \{\wt{W}_i\}_{i = 1}^{\ell + 1}.
    \end{gather*}
    Therefore, it suffices to analyze the distribution of $\prod_{j = i}^1 D_j \wt{W}_j x$. Again, we condition on the following event:
    \begin{equation*}
        \forall i \in [\ell]: \Tr D_i \geq \frac{d_i}{3}
    \end{equation*}
    which occurs with probability at least $1 - \delta / 8$. As in the proof of \cref{lem:f_grad_conc}, we observe the following distributional equivalence:
    \begin{gather*}
        \forall i \in [\ell]: \norm*{\prod_{j = i}^1 D_j \wt{W}_j (x)} \overset{d}{=} \norm*{\prod_{j = i}^1 W^\dagger_j x} \text{ where } \forall j \in \{2, \dots, i\} \in W^\dagger_j \in \R^{\Tr D_j \times \Tr D_{j - 1}},\ W^\dagger_1 \in \R^{\Tr D_1 \times d} \\
        \forall j \in \{2, \dots, i\} (W^\dagger_j)_{k, :} \thicksim \mc{N} \lprp{0, I / d_{j - 1}}, (W^\dagger_1)_{k, :} \thicksim \mc{N} (0, I / d).
    \end{gather*}
    A recursive application of \cref{thm:tsirelson} as in the proof of \cref{lem:f_grad_conc} yields:
    \begin{equation*}
        \norm*{\prod_{j = i}^1 D_j \wt{W}_j x} \geq \lprp{\frac{1}{2}}^i
    \end{equation*}
    with probability at least $1 - \delta / 16\ell^2$. A union bound over the $j$ layers concludes the proof of the first claim of the lemma.
    % \begin{align*}
    %     \norm*{\prod_{j = i}^1 D_j \wt{W}_j x} &\geq \frac{1}{2} \cdot \sqrt{\frac{d_i}{d_{i - 1}}}\norm*{\prod_{j = i - 1}^1 D_j \wt{W}_j x} && \text{Conditioning on } \prod_{j = i - 1}^1 D_j \wt{W}_j x \\ &\geq \lprp{\frac{1}{2}}^i \sqrt{d_i} && \text{By induction with probability at least } 1 - \delta / (8\ell).
    % \end{align*}
    % A union bound over the $j$ layers concludes the proof of the first claim of the lemma.

    % We will establish the second claim through a gridding based argument with some subtleties. Namely, we construct a new grid over the image of $\mb{B}(x,R)$ whenever the number of units in a hidden layer drops. With this outline in mind, we start by splitting our neural network into a series of segments. We define these segments inductively as follows:
    % \begin{equation*}
    %     i_1 = \ell, \qquad i_{j + 1} \coloneqq \argmin_{j < i_j} d_j
    % \end{equation*}
    % with segments implicitly defined by indices $\{i_j\}_{j = 1}^m$. Note $m \leq \ell$ and for $i_{j + 1} < i < i_j$, we have $d_i \geq d_{i_{j + 1}}$. We now establish the following claim inductively:
    We will establish the second claim through a gridding based argument with some subtleties. Namely, we construct a new grid over the image of $\mb{B}(x,R)$ whenever the number of units in a hidden layer drops lower than all the previous layers in the network starting from the input layer. These layers are precisely defined by the indices $i_j$ in \ref{eq:nn_dec}. We now establish the following claim inductively.
    \begin{claim}
        \label{clm:per_segmend_sp}
        Suppose for $j > 1$:
        \begin{equation*}
            \forall y \in f_{i_j} (\mb{B} (x, R)): \norm{f_{i_j}(x) - f_{i_j} (y)} \leq \wt{R}.
        \end{equation*}
        Then:
        \begin{gather*}
            \forall i \in \{i_j + 1, \dots, i_{j - 1} - 1\}, y \in
            \mb{B} (x, R): \norm{f_i (x) - f_i (y)} \leq \lprp{C \log
            \dmax}^{(i - i_j) / 2} \cdot \sqrt{\frac{d_i}{d_{i_j}}}
            \cdot \wt{R}, \\
            \forall y \in \mb{B} (x, R): \norm{\wt{f}_{i_{j-1}} (x) -
            \wt{f}_{i_{j-1}} (y)}  \cdot \leq \lprp{C \log \dmax}^{(i_{j - 1} - i_j) / 2} \cdot \wt{R}
        \end{gather*}\ynote{fill bounds on $R, \wt{R}$}
        with probability at least $1  - \delta / 8l$.
    \end{claim}
    \begin{proof}
        We start by constructing an $\eps$-net \cite[Definition 4.2.1]{vershynin}, $\mc{G}$, of $f_{i_j} (\mb{B} (x, R))$ with $\eps = \epsnetres$. Note that we may assume $\abs{\mc{G}} \leq (6 R / \eps)^{d_{i_j}}$. We will prove the statement on the grid and extend to rest of the space. For layer $i + 1$, we have $\forall y \in \mc{G}$:
        \begin{align*}
            \norm{\wt{f}_{i + 1, i_j} (\wt{x}) - \wt{f}_{i + 1, i_j} (y)} &= \norm{W_{i + 1} (f_{i, i_j}(\wt{x}) - f_{i, i_j}(y))} \leq \norm{f_{i, i_j}(\wt{x}) - f_{i, i_j}(y)} \cdot \sqrt{\frac{d_{i + 1}}{d_i}} \cdot \lprp{1 + \sqrt{\frac{\log 1 / \delta^\prime}{d_{i + 1}}}}
        \end{align*}
        with probability at least $1 - \delta^\prime$ as before by Tsirelson's inequality. By setting $\delta^\prime = \delta / (16 \abs{\mc{G}} \ell^2)$ and noting that $d_i \geq d_{i_j}$, the conclusion holds for layer $i + 1$ on $\mc{G}$ with probability at least $1 - \delta / (16\ell^2)$. By induction and the union bound, we get:
        \begin{gather*}
            \forall i \in \{i_j + 1, \dots , i_{j - 1} - 1\}, y \in \mc{G}: \norm{\wt{f}_{i, i_j} (y) - \wt{f}_{i, i_j}(\wt{x})} \leq (C \log \dmax)^{(i - i_j) / 2} \cdot \sqrt{\frac{d_i}{d_{i_j}}} \cdot \wt{R} \\
            \forall y \in \mc{G}: \norm{\wt{f}_{i_{j - 1}, i_j} (y) - \wt{f}_{i_{j - 1}, i_j}(\wt{x})} \leq \lprp{C \log \dmax}^{(i_{j - 1} - i_j) / 2} \cdot \wt{R}
        \end{gather*}
        with probability at least $1 - \delta / (16\ell^2)$. To extend
        to all $y \in \mc{G}$, we condition on the conclusion of
        \cref{lem:w_spec_conc} for all $W_i$ with $i \leq i_{j - 1}$ and
        note that $\forall y \in \mb{R}^{d_{i_j}}$,
        for $\wt{y} = \argmin_{z \in \mc{G}} \norm{z - y}$, 
        and for $i_j+1\le i<i_{j-1}$,
        \begin{align*}
            \norm{\wt{f}_{i, i_j} (\wt{x}) - \wt{f}_{i, i_j} (y)} &\leq \norm{\wt{f}_{i, i_j} (\wt{x}) - \wt{f}_{i, i_j} (\wt{y})} + \norm{\wt{f}_{i, i_j} (y) - \wt{f}_{i, i_j} (\wt{y})} \\
            &\leq \norm{\wt{f}_{i, i_j} (\wt{x}) - \wt{f}_{i, i_j}
            (\wt{y})} + \norm{y - \wt{y}} \prod_{k = i_{j} + 1}^i
            \norm{W_k} \\
            &\leq \norm{\wt{f}_{i, i_j} (\wt{x}) - \wt{f}_{i, i_j}
            (\wt{y})} + \epsilon \prod_{k = i_{j} + 1}^i
            \left(C\sqrt{\frac{d_k}{d_{k-1}}}\right) \\
            &= \norm{\wt{f}_{i, i_j} (\wt{x}) - \wt{f}_{i, i_j}
            (\wt{y})} + \epsilon C^{i-i_j}
            \sqrt{\frac{d_i}{d_{i_j}}},
        \end{align*}
        using that $d_i\ge d_{i_j}$ and assuming
        $d_{i_j}=\Omega(\log(1/\delta))$.
        Similarly, for $i=i_{j-1}$, we have
        \begin{align*}
            \norm{\wt{f}_{i_{j-1}, i_j} (\wt{x}) - \wt{f}_{i_{j-1}, i_j} (y)}
            &\leq \norm{\wt{f}_{i_{j-1}, i_j} (\wt{x}) -
            \wt{f}_{i_{j-1}, i_j}
            (\wt{y})} + \epsilon C^{i_{j-1}-i_j}
            \sqrt{\frac{d_{i_{j-1}-1}}{d_{i_j}}}.
        \end{align*}
        Since $\epsilon\le c\tilde R
        \sqrt{d_{i_j}/d_{i_{j-1}-1}}$, this concludes the proof of the
        claim.
    \end{proof}

    An inductive application of \cref{clm:per_segmend_sp}, a union bound and the observation that:
    \begin{equation*}
        \norm{f_i (x) - f_i (y)} \leq \norm{\wt{f}_i (x) - \wt{f}_i (y)}
    \end{equation*}
    concludes the proof of the lemma.
\end{proof}

\begin{lemma}
    \label{lem:x_i_anticonc}
    For all $i \in [\ell]$, we have:
    \begin{equation*}
        \#\lbrb{j: \abs{\inp{(W_{i + 1})_j}{x_i}} \geq \alpha_i
        \frac{\norm{x_i}}{\sqrt{d_i}}} \geq \lprp{1 -
        2\sqrt{\frac{2}{\pi}}\alpha_i} d_{i + 1}
    \end{equation*}
    with probability at least $1 - \delta$, provided
    $d_{i+1}\alpha_i^2\ge \ln(l/\delta)$.
\end{lemma}
\begin{proof}
    Follows from the fact that $\Pr(|Z|\le c)\le c\sqrt{2/\pi}$ for
    $Z\sim N(0,1)$, plus a simple application of Heoffding's Inequality.
\end{proof}

\subsection{Proving Local Gradient Smoothness}
\label{ssec:local_grad_smooth}

In this section, we show that the gradient is locally smooth which will imply the existence of adversarial examples. Adopting notation from \ref{eq:nn_def} and \ref{eq:sp_not}, we observe the following gradient decomposition:
\begin{align*}
    \nabla f(x) - \nabla f(y) &= W_{\ell + 1} \prod_{i = \ell}^1 D_i(x) W_i - W_{\ell + 1} \prod_{i = \ell}^1 D_i(y) W_i = W_{\ell + 1} \lprp{\prod_{i = \ell}^1 D_i(x) W_i - \prod_{i = \ell}^1 D_i(y) W_i} \\
    &= W_{\ell + 1} \lprp{\prod_{i = \ell}^1 D_i(x) W_i - (D_\ell(x) + (D_\ell (y) - D_\ell (x))) W_\ell\prod_{i = \ell - 1}^1 D_i(y) W_i} \\
    &= W_{\ell + 1} \lprp{D_\ell (x) W_\ell \lprp{\prod_{i = \ell - 1}^1 D_i(x) W_i - \prod_{i = \ell - 1}^1 D_i(y)W_i} + (D_\ell (y) - D_\ell (x)) W_\ell \prod_{i = \ell - 1}^1 D_i(y) W_i} \\
    &= \sum_{j = 1}^\ell W_{\ell + 1} \lprp{\prod_{i = \ell}^{j + 1} D_i(x) W_i}\cdot (D_j(y) - D_j(x)) W_j \cdot \lprp{\prod_{k = j - 1}^1 D_i(y) W_i} \tag{GD-DECOMP} \label{eq:grad_decomp}.
\end{align*}

Therefore, it suffices to bound each of the terms in expansion. Before
we proceed, we prove a structural lemma on the spectral norm of the
matrices appearing in the right-hand-side of the final expression in
\ref{eq:grad_decomp}. This will use the partitioning of the network as
in \cref{lem:scale_pres_ml} where the first layer in each segment is
the narrowest. We introduce some notation: for $i>j$, define
\begin{equation*}
    M_{i, j} (y) = \prod_{k = i}^{j + 1} D_k (y) W_k
\end{equation*}
and state and prove the lemma below:
\begin{lemma}
    \label{lem:nn_part_spec_bnd}
    We have:
    \begin{equation*}
        \forall \norm{y - x} \leq R, j \in [m]: \norm*{M_{i_j, i_{j + 1}} (y)} \leq (C \cdot \ell \cdot \sqrt{\log \dmax})^{(i_j - i_{j + 1}) / 2}
    \end{equation*}
    with probability at least $1 - \delta$.
\end{lemma}
\begin{proof}
    To start, consider a fixed $j \in [m]$ and condition on the conclusion of \cref{lem:scale_pres_ml} upto level $i_{j + 1}$. Now, consider an $\eps$-net of $f_{i_{j + 1}} (\mb{B} (x, R))$, $\mc{G}$, with resolution $\eps = \epsnetres$. As before, $\abs{\mc{G}} \leq (\dmax)^{C\ell d_{i_{j + 1}}}$ for some constant $C$. We additionally will consider subsets
    \begin{equation*}
        \mc{S} = \lbrb{(S_k)_{k = i_j - 1}^{i_{j + 1} + 1}:
        S_k\subseteq[d_k],\, \abs{S_k} \leq 4 d_{i_{j + 1}}},\quad \mc{B} = \lbrb{(b_k)_{k = i_j - 1}^{i_{j + 1} + 1}: b_k \in \{0, 1\}}.
    \end{equation*}
    Note that $\abs{\mc{G}} \cdot \abs{\mc{S}}^2 \cdot \abs{\mc{B}} \leq (\dmax)^{Cld_{i_{j + 1}}}$. For $y \in \mc{G}, S^1, S^2 \in \mc{S}, b \in \mc{B}$, consider the following matrix:
    \begin{equation*}
        M^{i_{j}, i_{j + 1}}_{y, S^1, S^2, b} = \prod_{k = i_{j}}^{i_{j + 1} + 1} ((\bm{1}\{b_k = 1\} D_k (y) + \bm{1} \{b_k = 0\} (D_{S^1_k} - D_{S^2_k})) W_k) \text{ where } 
        (D_S)_{i, j} = 
        \begin{cases}
            1, \text{if } i = j \text{ and } i \in S \\
            0, \text{otherwise}
        \end{cases}.
    \end{equation*}
    We will bound the spectral norm of $M^{i_{j}, i_{j + 1}}_{y, S^1, S^2, b}$. Similar to \cref{lem:scale_pres_ml}, observe that:
    \begin{equation*}
        M^{i_{j}, i_{j + 1}}_{y, S^1, S^2, b} \overset{d}{=} \prod_{k = i_{j}}^{i_{j + 1} + 1} ((\bm{1}\{b_k = 1\} D_k + \bm{1} \{b_k = 0\} (D_{S^1_k} - D_{S^2_k})) W_k) \text{ where }
        (D_k)_{i,j} = 
        \begin{cases}
            1, \text{with probability } \frac{1}{2} \text{ if } i = j\\
            0, \text{otherwise}
        \end{cases}.
    \end{equation*}
    To bound the spectral norm, let $\norm{v} = 1$ and we now have:
    \begin{align*}
        \norm{v^\top M^{i_j, i_{j + 1}}_{y, S^1, S^2, b}} &\leq \norm*{v^\top W_{i_j} \prod_{k = i_j - 1}^{i_{j + 1} + 2} ((\bm{1}\{b_k = 1\} D_k + \bm{1} \{b_k = 0\} (D_{S^1_k} - D_{S^2_k})) W_k)} \cdot \lprp{1 + \sqrt{\frac{\log \ell / \delta^\prime}{d_{i_{j + 1}}}}} \\
        &\leq \norm{v^\top W_{i_j}} \prod_{k = i_{j} - 1}^{i_{j + 1}} \lprp{1 + \sqrt{\frac{\log 1 / \delta^\prime}{d_{k}}}}
    \end{align*}
    with probability at least $\ell \delta^\prime$. But setting $\delta^\prime = \delta / (16 \cdot \abs{\mc{G}} \cdot \abs{\mc{S}} \cdot \abs{\mc{B}})$ yields with probability at least $1 - \delta /16$:
    \begin{equation*}
        \forall y \in \mc{G}, S_1, S_2 \in \mc{S}, b \in \mc{B}:
        ??? \norm{W_{i_j}} \cdot (C \cdot \ell \cdot \sqrt{\log \dmax})^{(i_j - i_{j + 1}) / 2}.
    \end{equation*}
    A bound on the spectral norm of $W_{i_j}$ concludes the bound for all $y \in \mc{G}$. For $y \notin \mc{G}$, we have with probability at least $1 - \delta$:
    \begin{equation*}
        \forall i \in \{i_j, \dots, i_{j + 1} + 1\}: \Tr \abs{D_i(y) -
        D_i(\wt{y})} \leq 4d_{i_{j+1}} \text{ where } \wt{y} = \argmin_{z \in \mc{G}} \norm{y - z} \ynote{Add a proof by conditioning.}
    \end{equation*}
\end{proof}

We proceed to do so in the following lemma:
\begin{lemma}
    \label{lem:ind_error_bnd}
    We have:
    \begin{equation*}
        \forall \norm{x - y} \leq R, j \in [\ell]: \norm*{W_{\ell + 1} \lprp{\prod_{i = \ell}^{j + 1} D_i(x) W_i}\cdot (D_j(y) - D_j(x)) W_j \cdot \lprp{\prod_{k = j - 1}^1 D_i(y) W_i}} \leq o(1)\ynote{fill}
    \end{equation*}
    with probability at least $1 - \delta$.
\end{lemma}
\begin{proof}
    Consider a fixed term in the decomposition of the gradient difference from \ref{eq:grad_decomp}; that is, consider the random vector-valued function:
    \begin{equation*}
        \gddiff_j(y) \coloneqq W_{\ell + 1} \lprp{\prod_{i = \ell}^{j + 1} D_i(x) W_i} \cdot (D_j(y) - D_j(x)) W_j \cdot \lprp{\prod_{k = j - 1}^1 D_i(y) W_i}.
    \end{equation*}
    We will show with high probability that $\gddiff_j(y) = o(1)$ with high probability for all $\norm{x - y} \leq R$. This will then imply the lemma by an union bound and \ref{eq:grad_decomp}. Let $k$ be such that $i_k = \argmin_{m < j} d_m$. We will condition on the weights of the network up to layer $i_k$. Specifically, we will assume the conclusions of \cref{lem:scale_pres_ml,lem:nn_part_spec_bnd} up to layer $i_k$. Observe now that:
    \begin{gather*}
        W_{\ell + 1} \prod_{j = \ell}^{j + 1} D_i(x) W_i \overset{d}{=} \wt{W}_{\ell + 1} \prod_{j = \ell}^{j + 1} D_i \wt{W}_i \eqqcolon H \text{ where } \\
        (D_i)_{m, n} = 
        \begin{cases}
            1, &\text{with probability } 1/2 \text{ if } m = n \\
            0, &\text{otherwise}
        \end{cases},
        \{W_i\}_{i = j + 1}^{\ell + 1} \overset{d}{=} \{\wt{W}_i\}_{i = j + 1}^{\ell + 1}
    \end{gather*}
    Therefore, $H$ is a spherically-symmetric random vector and we condition on on the following high probability bound on its length:
    \begin{align*}
        \norm{H} &\leq \norm*{\wt{W}_{\ell + 1} \prod_{j = \ell}^{j + 2} D_i \wt{W}_i} \cdot \lprp{1 + \sqrt{\frac{\log 1 / \delta^\prime}{d_j}}} \leq \lprp{2}^{\ell + 1 - j}
    \end{align*}
    with probability at least $1 - \ell \delta^\prime$ and our bound on $\delta^\prime$\ynote{Be precise here.}. Observe that the distribution of $H$ remains spherically symmetric even after conditioning on the above event. As in the proof of \cref{lem:nn_part_spec_bnd}, let $\mc{G}$ be an $\eps$-net of $f_{i_k}(\mb{B} (x, R))$ with $\eps$ as in the proof of \cref{lem:nn_part_spec_bnd}. We now show a basic structural claim of how activations pattern differ across the various layers between a point and its closest approximation in $\mc{G}$:
    \begin{claim}
        \label{clm:grid_approx_act_patt}
        We have:
        \begin{equation*}
            \forall m \in \{i_{k - 1}, \dots, i_k\}, y \in f_{i_k} (\mb{B} (x, R)): \Tr \abs{D_m (\wt{f}_{m, i_k} (y)) - D_m (\wt{f}_{m, i_k} (\wt{y}))} \leq 4d_{i_k} \text{ where } \wt{y} = \argmin_{z \in \mc{G}} \norm{z - y}
        \end{equation*}
        with probability at least $1 - \delta^\prime / \ell^2$.
    \end{claim}
    \begin{proof}
        We start by conditioning on the conclusion of \cref{lem:gau_spec_conc} upto layer $i_{k - 1}$. Then:
        \begin{equation*}
            \forall m \in \{i_{k - 1}, \cdots, i_k\}, y \in f_{i_k} (\mb{B} (x, R)): \norm{\wt{f}_{m, i_{k}} (y) - \wt{f}_{m, i+k} (\wt{y})} \leq \eps \cdot \lprp{C \dmax}^{(m - i_k) / 2}.
        \end{equation*}
        Now, let $m \in \{i_{k - 1}, \cdots, i_k + 1\}$ and $y \in \mc{G}$. We have:
        \begin{multline*}
            \max_{z \text{ s.t } \norm{z - y} \leq \eps} \# \{i: \sign ((W_m)_i^\top f_{m - 1, i_k} (y)) \neq \sign ((W_m)_i^\top f_{m - 1, i_k} (z))\} \\
            \leq \# \{i: \exists z \text{ s.t } \norm{z - y} \leq \eps \text{ and } \sign ((W_m)_i^\top f_{m - 1, i_k} (y)) \neq \sign ((W_m)_i^\top f_{m - 1, i_k} (z))\}.
        \end{multline*}
        Defining
        \begin{equation*}
            W_i(y) \coloneqq \bm{1} \{\exists z \text{ s.t } \norm{z - y} \leq \eps \text{ and } \sign ((W_m)_i^\top f_{m - 1, i_k} (y)) \neq \sign ((W_m)_i^\top f_{m - 1, i_k} (z))\},
        \end{equation*}
        we get:
        \begin{align*}
            \P \lbrb{W_i(y) = 1} &\leq \P  \lbrb{(C \dmax)^{(m - i_k) / 2} \cdot \eps \cdot \norm{w_i} \geq \abs{\inp{w_i}{y}}} \\
            &\leq \P \lbrb{\norm{w_i} \geq 2} + \P \lbrb{2\eps (C \dmax)^{(m - i_k) / 2} \geq \abs{\inp{w_i}{y}}} \leq \eps \cdot (C \dmax)^{(m - i_k) / 2}.
        \end{align*}
        Therefore, we have:
        \begin{equation*}
            \P \lbrb{\sum_{i = 1}^{d_m} W_i(y) \geq 4d_{i_k}} \leq d_m^{4d_{i_k}} \cdot \lprp{\eps (C \dmax)^{(m - i_k) / 2}}^{4d_{i_k}}
        \end{equation*}
        and hence by the union bound:
        \begin{equation*}
            \P \lbrb{\exists y \in \mc{G}: \sum_{i = 1}^{d_m} W_i (y) \geq 4d_{i_k}} \leq (C\dmax)^{4 \ell d_{i_k}} \cdot \eps^{4 d_{i_k}} \leq \frac{\delta'}{16\ell^4}.
        \end{equation*}
    \end{proof}
    
    
    We now break into two cases depending on how $d_{j}$ compares to $d_{i_k}$ and handle them separately.
    
    \paragraph{Case 1:} $d_j \leq d_{i_k} \poly (\log^{\ell}\dmax)$\ynote{Be more precise}. In this case, define the sets $\mc{S}$ and $\mc{B}$ as follows:"
    \begin{equation*}
        \mc{S} = \lbrb{(S_m)_{m = i_k + 1}^{j - 1}: \abs{S_m} \leq 4\cdot d_{i_k}}, \qquad \mc{B} = \lbrb{(b_m)_{m = i_k + 1}^{j - 1}: b_m \in \{0, 1\}}.
    \end{equation*}
    Now, for $Q^1, Q^2 \subset [d_j], y \in \mc{H}, S^1, S^2 \in \mc{S}, b \in \mc{B}$, define the random vector:
    \begin{equation*}
        V^{j, k}_{y, Q^1, Q^2, S^1, S^2, b} = H (D_{Q^1} - D_{Q^2}) W_j \prod_{m = j - 1}^{i_k + 1} (\bm{1}\lbrb{b_m = 1} D_m (y) + \bm{1} \lbrb{b_k = 0} (D_{S^1_m} - D_{S^2_m})) W_m.
    \end{equation*}
    Note that as before:
    \begin{equation*}
        V^{j, k}_{y, Q^1, Q^2, S^1, S^2, b} \overset{d}{=} H (D_{Q^1} - D_{Q^2}) W_j \prod_{m = j - 1}^{i_k + 1} (\bm{1}\lbrb{b_m = 1} D_m + \bm{1} \lbrb{b_m = 0} (D_{S^1_m} - D_{S^2_m})) W_m.
    \end{equation*}
    Note that $2^{d_{i_k}}\cdot \abs{G} \cdot \abs{S}^2 \cdot \abs{\mc{B}} \leq (\dmax)^{C \ell d_{i_k}}$. We now get:
    \begin{align*}
        \norm{V^{j, k}_{y, Q^1, Q^2, S_1, S_2, b}} &\leq \norm*{H (D_{Q^1} - D_{Q^2}) W_j \prod_{m = j - 1}^{i_k + 2} (\bm{1}\lbrb{b_m = 1} D_m + \bm{1} \lbrb{b_m = 0} (D_{S^1_m} - D_{S^2_m})) W_m} \cdot \lprp{1 + \sqrt{\frac{\log 1 / \delta^\dagger}{d_{i_k}}}} \\
        &\leq \norm{H (D_{Q^1} - D_{Q^2})} \cdot \prod_{m = i_k + 1}^{j} \lprp{1 + \sqrt{\frac{\log 1 / \delta^\dagger}{d_{m - 1}}}} \leq \norm{H D_Q} \cdot (C \ell \log \dmax)^{(j - i_k) / 2}
    \end{align*}
    where the final inequality follows from the fact that $d_m \geq d_{i_k}$ and by setting $\delta^\dagger = \delta / (32 \cdot 4^{d_{i_k}} \cdot \abs{\mc{G}} \cdot \abs{\mc{S}}^2 \cdot \abs{\mc{B}})$. A union bound now implies that the previous conclusion holds for all $Q^1, Q^2 \subset [d_{i_k}], y \in \mc{G}, S^1, S^2 \in \mc{S}, b \in \mc{B}$. For the first term, we use the trivial bound:
    \begin{equation*}
        \norm{H (D_{Q^1} - D_{Q^2})} \leq \sqrt{\abs{Q^1} + \abs{Q^2}} \cdot \max_m \abs{H_m} \leq 2 \sqrt{\abs{Q^1} + \abs{Q^2}} \cdot  \sqrt{\frac{\norm{H}}{d_j} \cdot \log \dmax}.
    \end{equation*}
    with probability at least $1 - \delta$\ynote{Be more precise here}. Furthermore, we get from \cref{lem:x_i_anticonc,lem:scale_pres_ml}, for all $y \text{ s.t } \norm{y - x} \leq R$:
    \begin{align*}
        \Tr \abs{D_j (y) - D_j (x)} &\leq \#\lbrb{i: \abs{\inp{f_{j - 1} (x)}{(W_j)_i}} \leq \frac{\norm{f_{j - 1} (x)}}{\poly \log^\ell \dmax}} + \frac{\norm{\wt{f}_j (x) - \wt{f}_j (y)}^2}{\norm{f_{j - 1} (x)}^2}\cdot \poly \log^\ell \dmax \\
        &\leq \frac{d_j}{\poly \log^\ell \dmax} + \frac{\norm{\wt{f}_j (x) - \wt{f}_j (y)}^2}{\norm{f_{j - 1} (x)}^2}\cdot \poly \log^\ell \dmax \leq \frac{d_j}{\poly \log^\ell \dmax}.
    \end{align*}
    Hence, we get:
    \begin{equation*}
        \forall \norm{y - x} \leq R, \forall m \in \{i_k + 1, \dots, j - 1\}: \Tr \abs{D_j (y) - D_j (x)} \leq \frac{d_j}{\poly \log^\ell \dmax}, \Tr \abs{D_m (f_{i_k} (y)) - D_m (\wt{y})} \leq 4d
    \end{equation*}
    where $\wt{y} = \argmin_{z \in \mc{G}} \norm{z - f_{i_k} (y)}$. Our bounds on $\norm{H}$ now concludes the proof of the lemma in this case\ynote{Add references to the inequalities}.

    \paragraph{Case 2:} $d_j \geq d_{i_k} \poly \log^\ell \dmax$. As in the previous case, we start by defining the sets $\mc{S}, \mc{B}$:
    \begin{equation*}
        \mc{S} = \lbrb{(S_m)_{m = i_k + 1}^{j - 1}: \abs{S_m} \leq 4\cdot d_{i_k}}, \qquad \mc{B} = \lbrb{(b_m)_{m = i_k + 1}^{j - 1}: b_m \in \{0, 1\}}.
    \end{equation*}
    Now, for $y \in \mc{G}, S^1, S^2 \in \mc{S}, b \in \mc{B}$, consider the random matrix:
    \begin{gather*}
        M^{j, k}_{y, S^1, S^2, b} \coloneqq W_{j - 1} \prod_{m = j - 2}^{i_k + 1} (\bm{1} \{b_m = 1\} D_m (y) + \bm{1} \{b_m = 0\} (D_{S_m^1} - D_{S_m^2})) W_m \\
        M^{j, k}_{y, S^1, S^2, b} \overset{d}{=} \wt{W}_{j - 1} \prod_{m = j - 2}^{i_k + 1} (\bm{1} \{b_m = 1\} D_m + \bm{1} \{b_m = 0\} (D_{S_m^1} - D_{S_m^2})) \wt{W}_m.
    \end{gather*}
    We will bound the spectral norm of $M^{j,k}_{y, S^1, S^2, b}$ for all $y,S^1,S^2,b$ with high probability as follows. Let $\mc{V}$ be a $1/9$-grid of $\mb{S}^{d_{i_k}}$ and $v \in \mc{V}$. We have:
    \begin{align*}
        \norm*{M^{j, k}_{y, S^1, S^2, b}v} &\leq \sqrt{\frac{d_{j - 1}}{d_{j - 2}}} \cdot \lprp{1 + \sqrt{\frac{\log 1 / \delta^\dagger}{d_{j - 1}}}} \cdot \norm*{\prod_{m = j - 2}^{i_k + 1} (\bm{1} \{b_m = 1\} D_m + \bm{1} \{b_m = 0\} (D_{S_m^1} - D_{S_m^2})) \wt{W}_m v} \\
        &\leq \sqrt{\frac{d_{j - 1}}{d_{i_k}}} \cdot \prod_{m = i_k + 1}^{j - 1} \lprp{1 + \sqrt{\frac{\log 1 / \delta^\dagger}{d_m}}} \leq \sqrt{\frac{d_{j - 1}}{d_{i_k}}} \cdot \lprp{C \ell \log \dmax}^{(j - i_k + 1) / 2}
    \end{align*}
    where the final inequality follows by the fact that $d_m \geq d_{i_k}$ and by setting $\delta^\dagger = \delta / (32 \cdot \ell \cdot \abs{\mc{G}} \cdot \abs{\mc{S}}^2 \cdot \abs{\mc{B}} \cdot \mc{V})$. By a union bound, the bound on the spectral norms of $M^{j,k}_{y, S^1, S^2, b}$ follows. We now condition on this event and the conclusion of \cref{lem:scale_pres_ml} up to layer $j - 1$ for the rest of the proof. 

    Let $\wt{M}^{j,k}_{y, S^1, S^2, b} = D_{j - 1}(y) \cdot M^{j,k}_{y, S^1, S^2, b}$ and for $y \in \mc{G}$, let $\wt{y} = f_{j - 1, i_k} (y)$ and $\wt{x} = f_{j - 1} (x)$. We have by an application of \cref{lem:large_width_proof_gd_diff_bnd} and a union bound over all $y \in \mc{G}, S^1, S^2 \in \mc{S}, b \in \mc{B}$:
    \begin{equation*}
        \forall y \in \mc{G}, S^1, S^2 \in \mc{S}, b \in \mc{B}: \norm{H^\top (D_j (y) - D_j (x)) \wt{M}^{j,k}_{y, S^1, S^2, b}} \leq o(1)
    \end{equation*}
    with probability at least $1 - \delta'/\ell^2$.
    
    % We obtain:
    % \begin{multline*}
    %     \norm*{H (D_j(\wt{y}) - D_j (\wt{y})) W_j \wt{M}^{j, k}_{y, S^1, S^2, b}} \\
    %     \leq \norm*{H (D_j(\wt{y}) - D_j (\wt{y})) W_j \mc{P}_V \wt{M}^{j, k}_{y, S^1, S^2, b}} + \norm*{H (D_j(\wt{y}) - D_j (\wt{y})) W_j \mc{P}_V^\perp \wt{M}^{j, k}_{y, S^1, S^2, b}}
    % \end{multline*}
    % Each of the two terms in the above expression is at most $1 / \poly \log^\ell \dmax$ from first analysis in the one layer case\ynote{Formalize this fully. Use spherical symmetry in the orthogonal setting and small scale when in $V$}. 
    
    To conclude the proof, we show by a simple union bound that for all $T \subset [d_{j}]$ such that $\abs{T} \leq 4d_{i_k}$ and all $y \in \mc{G}, S^1, S^2 \in \mc{S}, b \in \mc{B}$:
    \begin{equation*}
        \norm*{H D_T \wt{W}_j \wt{M}^{j,k}_{y, S^1, S^2, b}} = o \lprp{\frac{1}{\poly \log^\ell \dmax}}.
    \end{equation*}
    The lemma now follows from the previous two displays and \cref{clm:grid_approx_act_patt}.
\end{proof}

\begin{lemma}
    \label{lem:large_width_proof_gd_diff_bnd}
    Let $L, R, r > 0, k,m,n \in \mb{N}, M \in \mb{R}^{m \times n}$ such that $m \geq n$. Furthermore, suppose $W \in \mb{R}^{k \times m}$ and $H$ is distributed as follows:
    \begin{equation*}  
        W = 
        \begin{bmatrix}
            w_1^\top \\
            w_2^\top \\
            \vdots \\
            w_k^\top
        \end{bmatrix}
        \text{ with }
        w_i \overset{i.i.d}{\thicksim} \mc{N} (0, I / m), 
        \text{ and } H \thicksim \mathrm{Unif} (L\cdot \mb{S}^{k - 1}).
    \end{equation*}
    Furthermore, suppose $x \in \mb{R}^d$ satisfies $\norm{x} \geq R$ and $y$ be such that $\norm{y - x} \leq r$. Then:
    \begin{gather*}
        \mb{P} \lbrb{\norm{H^\top D W M} \geq 1024 \cdot \norm{M} \cdot \lprp{\sqrt{L \cdot \frac{r}{R} \log 2R/r \cdot \lprp{1 + \frac{\log 1 / \delta^\dagger}{m}}} + \frac{L}{k} \cdot \lprp{1 + \frac{\log 1 / \delta^\dagger}{m}}}} \leq \delta^\dagger \\
        \text{ where } D_{i,j} = 
        \begin{cases}
            0, & \text{if } i \neq j \\
            \bm{1} \lbrb{w_i^\top x \geq 0} - \bm{1} \lbrb{w_i^\top y \geq 0}, & \text{otherwise}
        \end{cases}.
    \end{gather*}
\end{lemma}
\begin{proof}
    Note that it suffices to analyze the random variable:
    \begin{equation*}
        \wt{H}^\top D W M \text{ for } \wt{H} \thicksim \mc{N} (0, 2L \cdot I / k).
    \end{equation*}
    Let $V$ denote the two-dimensional subspace of $\mb{R}^k$ containing $x,y$. We now decompose the norm as follows:
    \begin{equation}
        \label{eq:diff_decomp}
        \norm{\wt{H}^\top D W M} \leq \norm{\wt{H}^\top D W \proj_V M} + \norm{\wt{H}^\top D W \proj_V^\perp M} \leq \norm{\wt{H}^\top D W \proj_V}\cdot \norm{M} + \norm{\wt{H}^\top D W \proj_V^\perp M}.
    \end{equation}
    To apply Bernstein's inequality, we first expand on the first term:
    \begin{align*}
        \wt{H}^\top D W \proj_V = \sum_{i = 1}^k \wt{H}_i D_{i,i} \proj_V w_i.
    \end{align*}
    Letting $Z_i = \wt{H}_i D_{i,i} \proj_V w_i$, we note that $\E [Z_i] = 0$ and bound its even moments as follows:
    \begin{align*}
        \E \lsrs{\inp{v_j}{Z_i}^2} &= \E \lsrs{\wt{H}_i^2 \cdot D_{i,i}^2 \cdot \inp{v_j}{w_i}^2} \leq \frac{2L}{k} \cdot \E \lsrs{\norm{\proj_V w_i}^2} \cdot \P \lbrb{D_{i,i} \neq 0} = \frac{2L}{k} \cdot \frac{2}{m} \cdot \P \lbrb{D_{i,i} \neq 0} \\
        \E \lsrs{\inp{v_j}{Z_i}^\ell} &= \E \lsrs{\wt{H}_i^\ell \cdot D_{i,i}^\ell \cdot \inp{v_j}{w_i}^\ell} \leq (\ell - 1)!! \lprp{\frac{2L}{k}}^{\ell / 2} \cdot \E \lsrs{\norm{\proj_V w_i}^\ell} \cdot \P \lbrb{D_{i,i} \neq 0} \\
        &\leq (\ell - 1)!! \lprp{\frac{2L}{k}}^{\ell / 2} \cdot \lprp{2^{\ell / 2} \cdot \E \lsrs{\inp{w_i}{v_1}^\ell + \inp{w_i}{v_2}^\ell}} \cdot \P \lbrb{D_{i,i} \neq 0} \\
        &= 2\cdot (\ell - 1)!! \lprp{\frac{4L}{k}}^{\ell / 2} \cdot \E \lsrs{\inp{w_i}{v_1}^\ell} \cdot \P \lbrb{D_{i,i} \neq 0} = 2 \cdot ((\ell - 1)!!)^{2} \lprp{\frac{4L}{km}}^{\ell / 2} \cdot \P \lbrb{D_{i,i} \neq 0} \\
        &\leq 2 \cdot \ell! \cdot \lprp{\frac{8L}{km}}^{\ell / 2} \cdot \P \lbrb{D_{i,i} \neq 0}.
    \end{align*}
    For odd $\ell \geq 3$ we have by a similar manipulations:
    \begin{align*}
        \E \lsrs{\abs{\inp{v_j}{Z_i}}^\ell} &= \E \lsrs{\abs*{\wt{H}_i^\ell \cdot D_{i,i}^\ell \cdot \inp{v_j}{w_i}^\ell}} \leq \P \lbrb{D_{i,i} \neq 0} \cdot \E \lsrs{\abs{\wt{H}_i^\ell \cdot \norm{\proj_V w_i}^\ell}} \\
        &\leq \P \lbrb{D_{i,i} \neq 0} \cdot \sqrt{\E \lsrs{\lprp{\wt{H}_i \cdot \norm{\proj_V w_i}}^{2\ell}}} \leq \P \lbrb{D_{i,i} \neq 0} \cdot \sqrt{2 \cdot (2\ell)! \cdot \lprp{\frac{8L}{km}}^{\ell}} \\
        &\leq \P \lbrb{D_{i,i} \neq 0} \cdot \sqrt{2 \cdot (2\ell)!} \cdot \lprp{\frac{8L}{km}}^{\ell / 2} \leq \P \lbrb{D_{i,i} \neq 0} \cdot 2^\ell \ell! \cdot \lprp{\frac{8L}{km}}^{\ell / 2} \\
        &\leq \P \lbrb{D_{i,i} \neq 0} \cdot \ell! \cdot \lprp{\frac{32L}{km}}^{\ell / 2}
    \end{align*}
    By a union bound and an application of \cref{thm:bernstein} gives:
    \begin{equation*}
        \norm*{\sum_{i = 1}^k Z_i} \leq 2\max_{j \in \{1,2\}} \abs*{\sum_{i = 1}^k \inp{v_j}{Z_i}} \leq 256 \cdot \lprp{\sqrt{\frac{L}{m} \cdot \P \lbrb{D_{i,i} \neq 0} \cdot \log 1 / \delta'} + \frac{L}{km} \cdot \log 1 / \delta'}
    \end{equation*}
    with probability at least $1 - \delta'$ via a union bound. 

    For the other term in \cref{eq:diff_decomp}, we use $U$ to denote the left singular subspace of $M$ and $Y$ to denote the left singular vectors of $\proj_V^\perp \proj_U$ with non-zero singular values. Noting $\norm{\proj_V^\perp \proj_U} \leq 1$, we now have:
    \begin{equation*}
        \norm{\wt{H}^\top D W \proj_V^\perp M} \leq \norm{M} \cdot \norm{\wt{H}^\top D W \proj_V^\perp \proj_U} \leq \norm{M} \cdot \norm{\wt{H}^\top DW \proj_U}.
    \end{equation*}
    We expand the term on the right as follows:
    \begin{equation*}
        \wt{H}^\top D W \proj_U = \sum_{i = 1}^k \wt{H}_i D_{i,i} \proj_U w_i = \sum_{i = 1}^k D_{i,i} \cdot \lprp{\wt{H}_i \proj_U w_i} \eqqcolon Y_i.
    \end{equation*}
    Note $\wt{H}_i \proj_U w_i$ and $D_{i,i}$ are independent random variables (due to $\proj_V w_i$ and $\proj_V^\perp w_i$ being independent). Now, let $u \in \mrm{Span} (U) \text{ s.t }\norm{u} = 1$ and we bound the directional even moments of $Y_i$ with the aim of applying Bernstein's inequality as before:
    \begin{align*}
        \E \lsrs{\inp{u}{Y_i}^2} &= \E \lsrs{D_{i,i}^2 \cdot \wt{H}_i^2 \cdot \inp{u}{w_i}^2} = \frac{2L}{k} \cdot \frac{1}{m} \cdot \P \lbrb{D_{i,i} \neq 0} \\
        \E \lsrs{\inp{u}{Y_i}^\ell} &= \E \lsrs{D_{i,i}^\ell \cdot \wt{H}_i^\ell \cdot \inp{u}{w_i}^\ell} = \lprp{(\ell - 1)!!}^2 \cdot \lprp{\frac{2L}{km}}^{\ell / 2} \cdot \P \lbrb {D_{i,i} \neq 0} \leq \ell! \cdot \lprp{\frac{2L}{km}}^{\ell / 2} \cdot \P \lbrb{D_{i,i} \neq 0}.
    \end{align*}
    Similarly, for odd $\ell \geq 3$, we have:
    For odd $\ell \geq 3$ we have by a similar manipulations:
    \begin{align*}
        \E \lsrs{\abs{\inp{u}{Y_i}}^\ell} &= \E \lsrs{\abs*{\wt{H}_i^\ell \cdot D_{i,i}^\ell \cdot \inp{u}{w_i}^\ell}} \leq \P \lbrb{D_{i,i} \neq 0} \cdot \E \lsrs{\abs{\wt{H}_i^\ell \cdot \inp{u}{w_i}^\ell}} \\
        &\leq \P \lbrb{D_{i,i} \neq 0} \cdot \sqrt{\E \lsrs{\abs{\wt{H}_i^\ell \cdot \inp{u}{w_i}^{2\ell}}}} \leq \P \lbrb{D_{i,i} \neq 0} \cdot \sqrt{(2\ell)! \cdot \lprp{\frac{2L}{km}}^{\ell}} \\
        &\leq \P \lbrb{D_{i,i} \neq 0} \cdot \sqrt{(2\ell)!} \cdot \lprp{\frac{2L}{km}}^{\ell / 2} \leq \P \lbrb{D_{i,i} \neq 0} \cdot 2^\ell \ell! \cdot \lprp{\frac{2L}{km}}^{\ell / 2} \\
        &\leq \P \lbrb{D_{i,i} \neq 0} \cdot \ell! \cdot \lprp{\frac{8L}{km}}^{\ell / 2}
    \end{align*}

    Now, consider a $1/3$-net of $\mc{G} \coloneqq \mrm{Span} (U) \cap \S^{m - 1}$, $\wt{\mc{G}}$ and we get for any $z \in \mrm{Span} (u)$:
    \begin{equation*}
        \norm{z} = \max_{u \in \mc{G}} \inp{u}{z} = \max_{u \in \mc{G}} \inp{u - \wt{u}}{z} + \inp{\wt{u}}{z} \leq \max_{u \in \mc{\wt{G}}} \inp{u}{z} - \frac{\norm{z}}{3} \implies \norm{z} \leq \frac{3}{2} \max_{u \in \mc{G}} \inp{u}{z}.
    \end{equation*}
    Note that since the rank of $\mrm{Span} (U)$ is at most $n$. We may assume $\abs{\mc{G}} \leq (30)^{n}$\ynote{cite}. By a union bound:
    \begin{equation*}
        \norm*{\sum_{i = 1}^n Y_i} \leq 2 \max_{u \in \mc{\wt{G}}} \inp*{u}{\sum_{i = 1}^n Y_i} \leq 256 \cdot \lprp{\sqrt{L \cdot \P \lbrb{D_{i,i} \neq 0} \cdot \lprp{1 + \frac{\log 1 / \delta'}{m}}} + \frac{L}{k} \cdot \lprp{1 + \frac{\log 1 / \delta'}{m}}}
    \end{equation*}
    with probability at least $1 - \delta'$. The lemma follows from the previous discussion and \cref{lem:mis_sign_prob} by picking $\delta' = \delta^\dagger / 4$ and applying a union bound.
\end{proof}


==> content/todo <==
1) 369 - Add factor of 2 - Done
2) 377 - Change m set to i_{j + 1} + 1 - Done
3) 385 - Remove -1 from m - 1 -i_{j + 1} - Done
4) Below 386: i_k -> i_{j + 1}, 4d_{i_j} -> 4d_{i_{j + 1}} - Done
5) 418 - Change max_m |H_m| to infinity norm - Done
6) 419 - Change to be more explicit with matrices set to vectors $e_i$ - Done
7) 420 - Comment on second term of the inequality - Done
8) 429 - Add the factor of 2 - Done
9) 435 - Add reference to the case - Done 
10) 442 - Add explanation after pointing to the current case - Done
11) 490 - Add explanation about blah is a Lipschitz function of blah - Done
12) 495 - Add square on right hand side and fix the 8 on the next line - Done
13) 496 - Similar to previous point - Done
14) 497 - Add some explanation (1 + x) < e^x < 1 + 2x for x small enough - Done
15) 512 - Change 128 to something like ~50, change f_{i - 1} (x) => f_{i - 1} (y) - Done
16) 513 - 519 - Replace 64\ell^2 d^3 by 16\ell^2 d^3 - Done
17) Change Proof of Lemma 2.1 to add the inductive hypothesis. Explicitly state that it is proven by induction on $m$ where in the second distributional equality, we use the inductive hypothesis by noting that the distribution of the prefix is independent of the last term. Maybe explain the third step too. - Done
18) Add a page before the main paper stating that the submission has been included to aid navigation - Done
